A New Approach to DDoS Defense using SDN and NFV

Networks today rely on expensive and proprietary hard- ware appliances, which are deployed at fixed locations, for DDoS defense. This introduces key limitations with respect to flexibility (e.g., complex routing to get traffic to these "chokepoints") and elasticity in handling changing attack patterns. We observe an opportunity to ad- dress these limitations using new networking paradigms such as software-defined networking (SDN) and network functions virtualization (NFV). Based on this observation, we design and implement of Bohatei, an elastic and flexible DDoS defense system. In designing Bohatei, we address key challenges of scalability, responsive- ness, and adversary-resilience. We have implemented defenses for several well-known DDoS attacks in Bohatei. Our evaluations show that Bohatei is scalable (handling 500 Gbps attacks), responsive (mitigating attacks within one minute), and resilient to dynamic adversaries.

==> adversary.tex <==
\section{ADVERSARIAL DDOS DEFENSE}
\label{sec:adversary}

In this section, we discuss potential vulnerabilities of \Name in an 
adversarial environment and present our strategies to combat them.
We consider an environment where an adversary may:

\begin{packeditemize}

\item change attack types $\attackindex$;

\item  change attack volume $\Traffic_{\edgepopindex,\attackindex}$ 
within a fixed total budget of attack traffic volume $B=
\sum\limits_{\edgepopindex}^{}
\sum\limits_{\attackindex}^{}
\Traffic_{\edgepopindex,\attackindex}$;

\item apply the above changes instantly at any point in time.

\end{packeditemize}

\seyed{must make the above consistent with \S\ref{subsec:threat_model}}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{System Reaction Latency}

The most relevant performance metric of \Name in an adversarial 
environment is the \emph{system reaction latency}, denoted by 
$\Delta_{\Name}$, which is the time interval between the time attack 
traffic first enters the ISP network to the time the orchestration layer 
has finished configuring the network with respect to the attack. To make
this concrete, let's consider the ISP-wide events in reaction to an 
attack:

\begin{packedenumerate}

\item Attack traffic enters the ISP network at time $t_0$;

\item \Classifier successfully classifies attack traffic and 
notifies the controller $t_1$;

\item Resource assignment (i.e., DSP and SSP) solutions 
are available at $t_2$;

\item Network orchestration is complete at time $t_3$.

\end{packedenumerate}

Then we have $\Delta_{\Name} = t_3 - t_0$. While we have carefully 
engineered the system as to minimize each above sub intervals 
$t_i - t_{i-1}$ ($i=2,3$) as discussed in previous sections, if the 
adversary changes the attack characteristics within $\Delta_{\Name}$ 
after $t_0$, \Name cannot react to the new attack in 
time.\footnote{The interval $t_1 - t_0$ is mostly taken by the 
network-wide traffic sampling scheme (e.g., NetFlow).}

We, therefore, 
consider a set of defense strategies for such adversarial cases.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Defense Strategies in an Adversarial Environment}

Below we discuss two defense strategies against the actions of an
strategies adversary that can quickly change attack type/volume.

\begin{packeditemize}

\item \emph{Deploying ``giant'' defense graph}: To defend against
an adversary that keeps changing the attack type with a frequency
smaller than $\Delta_{\Name}$, we use a conservative defense approach 
using which all traffic goes through a graph that is made of all individual 
logical graphs of all different attack types. As such, the appropriate 
sub-graph will catch the attack traffic. While this strategy is somewhat 
similar to the case of using a monolithic box as done today, it still 
surpasses monolithic box approach due to the scale-out
capability of \Name.

\item \emph{Overprovisioning}: To protect the customer against an
adversary that changes attack volumes frequently (i.e., in time intervals
smaller than $Delta_{\Name}$), we conservatively multiply 
$\vms_{\attackindex,\vertexindexi}^{\datacenterindex,\aserver}$ values
given by the resource assignment by an overprovisioning factor 
$\gamma > 1$ to create a cushion for sudden increase in attack volumes.
The parameter $\gamma$ can be determined by the SLA and depends 
on the maximum amount of resources that the ISP is willing to or 
capable of assigning to protecting the customer.

\end{packeditemize}

To defend an adversary that  can quickly change attack time and 
volume simultanously, \Name combines the above strategies. We 
evaluate these strategies in \S\ref{sec:evaluation}.

Note that the above strategies are to be used under the worst-case 
assumption that  the ISP does not know  and cannot learn the decision 
algorithm of the adversary. If this assumption does not hold, it is possible 
to do better by incorporate information about adversary's decision making 
into \Name (e.g., using moving weighted average values to predict 
future attack volumes).














==> concerns.tex <==
\section{Concerns}
\begin{itemize}

 \item just applied model checking etc  tools here. what’s the big deal?

 \item just found non-interesting errors, e.g., ip v6 gets dropped
 
 \item what is the  guarantee? what is covered/non covered? should we worry about non-covered parts?
 should i be happy if you tell things are fine based on some sampling/statistical testing?
 
 \item for each section, find the strawman solutions.
 
 \item what setting can we accommdate (enterprise, data center, cloud, interdomain, etc)? 
 are the principles  generalizable? 
 
 \item what do we envision as the end product? an open flow app? a new architecture? a set of
 apis like flowtags?\dots
 
 \item change of policy over time?
 
\end{itemize}


\comment{

\section{Macro Concerns}
\begin{itemize}

\item  why are prior testing abstractions like propositional logic, frenetic
formalism, hsa formalism not sufficient?

e.g., why is this not LTL/CTL or whatever from frenetic not enough -- we need to get some formal person to 
 look at this? 

%\item scalability?


%\item what is the criteria for a good test script? min time to run? 
%min number of entries? exploring the leaves in a certain order?

%\item interference from background?

\end{itemize}

\comment{
\section{Micro concerns}

\begin{itemize}

\item the test traffic generation logic runs at the controller. but how to tell a host to run certain traffic?

\item don't like to repeat the nsdi examples.

\item we can assume all mboxes are in state0 that allows everything. then static config takes it to state1.
this way even a packet filter will have a state machine.

\item the dpg is pictorially too high-level. where is the detailed policy represented?
e.g., block H2$\rightarrow$xyz.com rather that just FW H2?


\item what is the test gurantee/coverage? a simple example: suppose
a FW is suppose to drop packets destined to $ip_1$ and allow everything 
else. how do we test this? suppose the five tuple has $N$ bits. to ensure
there are no false pos/neg we need to test $2^N$ possibilities?

\item need to clearly define the traditional black hole, loop, and 
reachability in the presence of mboxes. e.g., is it considered a black 
hole when an ips drops packets?
is it a loop when an http response goes back from a cache to the host?
suppose there is a NAT between A and B; does this mean A can "reach" B?

\item (not a concern!) ATPG can be still orthogonally useful for exploring paths purely 
involving switches and routers.


\end{itemize} 
}
}

==> formulation/distributed/algorithms.tex <==
\section{Algorithms}

\subsection{DSP}
\begin{itemize}

\item We observe the following w.r.t. data center $\datacenter_\datacenterindex$: (1) its link capacity
$\capacity^{link}_{\datacenterindex}$ is \emph{attack type-independent}; (2) its compute capacity
$\capacity^{compute}_{\datacenterindex}$ is \emph{attack type-dependent} as specified by 
$\vms_\attackindex$.

\item {\bf Accommodating the primary goal of DSP:} The above observations combined with the fact that \
the primary goal of DSP is to minimize
$\traffic_{left}$ suggest that an algorithm to DSP should try to process as much volume of traffic
as possible. This means, the algorithm should try to get rid of the cheapest attack (i.e., attack with the
smallest $\vms_\attackindex$ value) first. Once all ISP-wide attack traffic of the cheapest type is
assigned to data center, the algorithm move on to the next cheapest attack type and so on. The
algorithm terminated once all attack traffic is assigned to data centers or we run out of data center 
resources.

\item {\bf Accommodating the secondary goal of DSP:} There may exist multiple ways of traffic to data 
center that yield the same $\traffic_{left}$ value, which means they are equally good w.r.t. the primary goal
of DSP. Given the secondary goal of DSP (i.e., minimizing the solution cost), among these solutions we 
want to choose the solution that achieves this minimum  $\traffic_{left}$ value at the minimum cost.

\item The above two paragraphs outline a natural hierarchical structure to design an algorithm to solve
DSP. An outer loop accommodates the primary DSP using a greedy approach (since it is identical to 
the fractional knapsack problem) by choosing the next cheapest attack type. For the current attack type
selected by the outer loop, the inner simply minimized the cost of accommodating that attack type. The
pseudocode is outlines in the following Listing.

\begin{codebox}
 \li Sort $\boldsymbol{\attack}$ in increasing order of $\vms_\attackindex$ values. 
 $\boldsymbol{\attack}' \gets [\attack_1',\dots, \attack_{\attackindex}',\dots, \attack_{\mid \boldsymbol{\attack} \mid}']$ is the sorted list.
 
 \li Sort cost values $\cost_{\edgepopindex,\datacenterindex}$ in increasing order and store them in list $\boldsymbol{\cost}'$
 
\li  \For $\attackindex' \gets 1$ to $\mid \boldsymbol{\attack} \mid$
\li \Do  \For $l' \gets 1$ to $\mid \boldsymbol{\cost'} \mid$	
\li \Do $\edgepopindex'  \gets \edgepopindex$ where $\boldsymbol{\cost}'[l']$ = $\cost_{\edgepopindex,\datacenterindex}$
\li $\datacenterindex'  \gets \datacenterindex$ where $\boldsymbol{\cost}'[l']$ = $\cost_{\edgepopindex,\datacenterindex}$
\li Assign as much of traffic $\Traffic_{\edgepopindex',\attackindex'}$ as possible to
data center $\datacenter_{\datacenterindex'}$
\li Update $\Traffic_{\edgepopindex',\attackindex'}$, $\capacity^{link}_{\datacenterindex'}$, and
$\capacity^{compute}_{\datacenterindex'}$ values as per the assignment
\li Terminate if all traffic is assigned or no assignment is possible
\End
\End
\end{codebox}

\item The above algorithm is optimal with time complexity 
$O(max(\mid \boldsymbol{\attack} \mid
\mid \boldsymbol{\edgepop} \mid
\mid \boldsymbol{\datacenter} \mid, 
\mid \boldsymbol{\edgepop} \mid
\mid \boldsymbol{\datacenter} \mid
lg(\mid \boldsymbol{\edgepop} \mid
\mid \boldsymbol{\datacenter} \mid
))$. The first element of $min$ is the cost of nested loops and
the second element represent the cost of sorting $\cost_{\edgepopindex,\datacenterindex}$
values.

\item Since the number of attack types is small, in practice, the time complexity is
$O(\mid \boldsymbol{\edgepop} \mid
\mid \boldsymbol{\datacenter} \mid
lg(\mid \boldsymbol{\edgepop} \mid
\mid \boldsymbol{\datacenter} \mid)$

\item We should say how frequently each part of code runs. E.g., sort is once in a while thing.

\end{itemize}

\subsection{SSP}

\begin{itemize}

\item In each data center, we have current information of servers capacity (i.e., how many new
VMs can be launched on each server of the data center).

\item Option 1: Since $\vms_\attackindex$ are small number ($\leq 5$), we can just assign each 
attack type to the best possible choice as defined in~\ref{subsec:ssp_def} using simple bin packing
heuristics like first-fit.

\item Option 2: We can do some fancy graph partitioning algorithm like Kernighan-Lin.

\end{itemize}


==> formulation/distributed/analysis.tex <==
\section{Analysis and Discussion}


==> formulation/distributed/macros_dist.tex <==
\newcommand{\edgepopindex}{\ensuremath{\mathit{e}}}
\newcommand{\edgepop}{\ensuremath{\mathit{E}}}
\newcommand{\attackindex}{\ensuremath{\mathit{a}}}
\newcommand{\attack}{\ensuremath{\mathit{A}}}
\newcommand{\datacenterindex}{\ensuremath{\mathit{d}}}
\newcommand{\datacenter}{\ensuremath{\mathit{D}}}
\newcommand{\traffic}{\ensuremath{\mathit{T}}}
\newcommand{\vms}{\ensuremath{\mathit{N}}}
\newcommand{\capacity}{\ensuremath{\mathit{C}}}
\newcommand{\cost}{\ensuremath{\mathit{L}}}
\newcommand{\fraction}{\ensuremath{\mathit{f}}}

%%%%%%%%%OLD STUFF%%%%%%%%%%%
%\comment{ 
\newcommand{\Traffic}{\ensuremath{\mathit{T}}}
\newcommand{\FootPrint}{\ensuremath{\mathit{F}}}
\newcommand{\Pop}{\ensuremath{\mathit{l}}}
\newcommand{\PopA}{\ensuremath{\mathit{l_\mathit{in}}}}
 \newcommand{\PopB}{\ensuremath{\mathit{l_\mathit{out}}}}
 \newcommand{\Attack}{\ensuremath{\mathit{A}}}
 \newcommand{\NumAttacks}{\ensuremath{\mathit{N}_\Attack}}
 \newcommand{\AttackIndex}{\ensuremath{\mathit{j}}}
 \newcommand{\Detection}{\ensuremath{\mathit{D}}}
 \newcommand{\NumDetection}{\ensuremath{\mathit{N}_\Detection}}
 \newcommand{\DetectionIndex}{\ensuremath{\mathit{d}}}
 \newcommand{\Classification}{\ensuremath{\mathit{C}}}
 \newcommand{\ClassificationIndex}{\ensuremath{\mathit{c}}}
 \newcommand{\NumClassification}{\ensuremath{\mathit{N}_\Classification}}
 \newcommand{\Response}{\ensuremath{\mathit{R}}}
 \newcommand{\ResponseIndex}{\ensuremath{\mathit{r}}}
 \newcommand{\NumResponse}{\ensuremath{\mathit{N}_\Response}}
 \newcommand{\CapacityInstances}{\ensuremath{\mathit{TotalInstances}}}
 \newcommand{\CapacityPerInstance}{\ensuremath{\mathit{Cap}}}
 \newcommand{\DetectionReqd}{\ensuremath{\mathit{DREQD}}}
 \newcommand{\ClassificationReqd}{\ensuremath{\mathit{CREQD}}}
 \newcommand{\ResponseReqd}{\ensuremath{\mathit{RREQD}}}
 \newcommand{\CRChain}{\ensuremath{\mathit{Chain}}}
 
 \newcommand{\ActiveInstance}{\ensuremath{\mathit{d}}}
 \newcommand{\TrafficFlow}{\ensuremath{\mathit{f}}}
 \newcommand{\Instance}{\ensuremath{\mathit{j}}}
 \newcommand{\InstanceToo}{\ensuremath{\mathit{j'}}}
 \newcommand{\InstanceThree}{\ensuremath{\mathit{j''}}}
 \newcommand{\Type}{\ensuremath{\mathit{Type}}}
 \newcommand{\Location}{\ensuremath{\mathit{Loc}}}
 \newcommand{\Load}{\ensuremath{\mathit{Load}}}
 \newcommand{\Chain}{\ensuremath{\mathit{Chain}}}
 \newcommand{\ChainLocation}{\ensuremath{\mathit{k}}}
%}

==> formulation/distributed/requirements.tex <==
\section{System requirements}

Our goal is three-fold:

\begin{itemize}

\item Decide how many {\em instances} of each type of detection, classification, and 
 response modules we need at each location. 

\item Set up the correct routing logic so that the classification and response chain is setup 
 correctly  and that the service chain is implemented correctly

\item Objectives: 
	\begin{itemize}
	\item minimize total latency on impact, 
	\item drop attack traffic as soon as possible,
	\item minimize network congestion as much as possible, 
	\item use as few instances as possible   to minimize total operating cost
	\end{itemize}
\end{itemize}


==> formulation/distributed/system.tex <==
\section{Problem Definition}

\subsection{Setup}

\begin{itemize}

\item {\bf Note 1:} For clarity, what we present here is with respect to one particular customer 
(it is trivial to extend it to the case of multiple customers).

\item {\bf Note 2:} We assume C (classification) is already completed, so now we can determine
attack traffic at the ingress.

\item {\bf Note 3:} We focus on the task of resource assignment to determine how many VMs and
where (i.e., which data centers and which machines inside the selected data centers) to launch
to implement A (analysis) and R (response).

\item {\bf ISP architecture:} As shown in Figure~\ref{fig:isp}, the ISP is composed of  a set of edge PoPs 
$\boldsymbol{\edgepop}=
\{\edgepop_1,\dots, \edgepop_{\edgepopindex},\dots, \edgepop_{\mid \boldsymbol{\edgepop} \mid}\}$, 
a set of data centers 
$\boldsymbol{\datacenter}=
\{\datacenter_1,\dots, \datacenter_{\datacenterindex},\dots, \datacenter_{\mid \boldsymbol{\datacenter} \mid}\}$, 
a global controller, and high-capacity backbone switches and links\footnote{We assume 
backbone switches and links do not cause congestion.}. The high-level role of the ISP is 
to transit traffic between its edge PoPs.

\begin{figure}[h]
\centering
\includegraphics[width=340pt]{figs/zoomout_view.pdf}
\tightcaption{ISP architecture.}
\label{fig:isp}
\end{figure}

\item {\bf Data center architecture:} Zooming into a data center $\datacenter_{\datacenterindex}$ 
shown in Figure~\ref{fig:data_center}, it is assumed to have a typical hierarchical topology of 
switches. 

\begin{figure}[h]
\centering
\includegraphics[width=280pt]{figs/zoomin_view.pdf}
\tightcaption{Data center architecture.}
\label{fig:data_center}
\end{figure}

\item The goal of the {\bf resource assignment problem} is to decide which servers are responsible 
for processing (i.e., running the required A and R modules) for the ISP-wide input attack traffic.

\item {\bf Challenges of a centralized solutions} The ILP formulation gives a globally optimal solution 
to the resource assignment problem. However, it is hindered by two serious problems: scalability and 
centrality. Besides being too slow, it is not practical to maintain all low-level (e.g., a VM swap 
out event on a server) in a centralized manner. We, therefore, aim to provide a natural distributed 
solution to this problem.

\item {\bf Distributed approach} We decompose the resource assignment problem into two natural
sub-problems:

{\bf (1) Data Center Selection Problem (DSP)}: Assigning input attack traffic to data centers.

{\bf (2) Server Selection Problem (SSP)}: Assigning servers inside each selected data center
(as given by DSP) to run the required A and R modules to process the assigned attack traffic.

\end{itemize}


\subsection{Data Center Selection Problem (DSP)}

\begin{itemize}

\item  {\bf Notataions:} Let  $\boldsymbol{\attack}=
\{\attack_1,\dots, \attack_{\attackindex},\dots, \attack_{\mid \boldsymbol{\attack} \mid}\}$
denote the set of possible DDoS attacks (e.g., SYN flood, NTP amplification).  
Further, let $\Traffic_{\edgepopindex,\attackindex}$ 
denote the total volume of attack traffic of type $\attackindex \in \boldsymbol{\attack}$ 
 at ingress $\edgepopindex \in \boldsymbol{\edgepop}$ destined to the customer. 
Note that $\Traffic_{\edgepopindex,\attackindex}$ requires to be ``dealt with''; (i.e., 
it needs to go through the required sequence of A and R modules at some data 
center(s).\footnote{Non-attack traffic is simply forwarded to the customer after 
traversing backbone links and switches (without going to any data center).} The cost 
of transferring each unit of traffic from ingress $\edgepopindex$ to data center 
$\datacenterindex$ is $\cost_{\edgepopindex,\datacenterindex}$. This cost represents 
the traffic footprint and latency associated with unit traffic.


\item {\bf Resource Constraints:} As stated before, we assume backbone links and switches 
do not cause bottleneck. However, a data center has limited link and compute capacity to 
assign to traffic. The traffic processing service that each data center
$\datacenter_\datacenterindex$ can provide is limited by two types of constraints: its current 
I/O link capacity (i.e., how much traffic the data center can transfer with the outside world) 
and its current computing capacity (i.e., what is the total available of compute capacity of its servers),
denoted by $\capacity^{link}_{\datacenterindex}$  and $\capacity^{compute}_{\datacenterindex}$,
respectively.  Each unit of traffic $\Traffic_{\edgepopindex,\attackindex}$ requires $\vms_\attackindex$
VMs (to implement the required A and R modules for attack type $\attackindex$).

\item A {\bf solution} to DSP involves: 

(1) A feasible assignment of attack traffics to data centers (i.e., selected data centers have 
enough link and compute capacity to deal the assigned traffic);

(2) A feasible assignment of servers inside selected data centers to run the required VMs to 
realize the required A and R modules for the incoming attack traffic. 

Note that input traffic volume $\Traffic_{\edgepopindex,\attackindex}$ can be split
and sent to different data centers. Let $\fraction_{\edgepopindex,\attackindex,\datacenterindex}$
show the fraction of traffic $\Traffic_{\edgepopindex,\attackindex}$ that a solutions decides to
send to data center $\datacenter_\datacenterindex$. 

\item The {\bf cost of a solution} is 
$\sum\limits_{\edgepopindex=1}^{\boldsymbol{\edgepop}} 
\sum\limits_{\datacenterindex=1}^{\boldsymbol{\datacenter}}
(\cost_{\edgepopindex,\datacenterindex} 
\times
\sum\limits_{\attackindex=1}^{\boldsymbol{\attack}}
\fraction_{\edgepopindex,\attackindex,\datacenterindex})$

\item The {\bf primary goal of a solution to DSP:} Let 
$\traffic_{total} = \sum\limits_{\edgepopindex=1}^{\boldsymbol{\edgepop}} 
\sum\limits_{\attackindex=1}^{\boldsymbol{\attack}}
\Traffic_{\edgepopindex,\attackindex}$
denote the  total attack traffic volume. Since data centers have limited capacity, in general,
a fraction of $\traffic_{total}$ may not be handled by data centers and, consequently, reach 
the customer. Let $\traffic_{handled}$ and $\traffic_{left}$ denote the volume of attack traffic 
the ISP handles and the volume of attack traffic that reaches the customer, respectively (i.e.,
$\traffic_{total} = \traffic_{handled}+\traffic_{left}$).
Formally,   $\traffic_{handled} = 
\sum\limits_{\edgepopindex=1}^{\boldsymbol{\edgepop}} 
\sum\limits_{\attackindex=1}^{\boldsymbol{\attack}}
(\Traffic_{\edgepopindex,\attackindex}
\times
\sum\limits_{\datacenterindex=1}^{\boldsymbol{\datacenter}}
\fraction_{\edgepopindex,\attackindex,\datacenterindex})$.
The primary goal of a solution is to minimize $\traffic_{left}$.
Note that the primary goal is defined irrespective of the solution cost.

\item The {\bf secondary goal of a solution to DSP:} Among all solutions that yield the 
minimum value of $\traffic_{left}$, we want to choose the solution with the lowest cost.

\end{itemize}

\subsection{Server Selection Problem (SSP)}
\label{subsec:ssp_def}

\begin{itemize}

\item Inside data center $\datacenter_{\datacenterindex}$, the total current compute capacity 
$\capacity^{compute}_{\datacenterindex}$ is composed of the sum of individual compute
capacities of its servers.

\item The {\bf goal of a solution to SSP:} is to localize the VMs that implement A and R of 
a given attack as much as possible. The following four possible choices at sorted in the 
order of decreasing locality: on the same server, under the same ToR switch, under the same 
aggregate switch, and under the same core switch.

\end{itemize}

%%%%%%%%%%%%%%%%OLD STUFF BELOW%%%%%%%%%%%%%%%%
\comment{
\item We have $\NumAttacks$ possible DDoS attacks; $\Attack_\AttackIndex$ with
$\AttackIndex = 1\dots\NumAttacks$   denotes a specific type of attack.  Let
$\Traffic_{\PopA,\PopB,\AttackIndex}$ denote the total volume of {\em potential
attack} traffic of type $\AttackIndex$ from ingress $\PopA$ to egress $\PopB$.
We say potential because we may not know how much of it will be true attack
until after the required classification modules have been applied.  These are
assumed to be non-overlapping; e.g.,  things like syn-flood, NTP reflector, DNS
amplifiction, or unknown.


\item We have $\NumDetection$ possible {\em attack detection} modules and
$\Detection_\DetectionIndex$ with $\DetectionIndex \in 1\dots\NumDetection$
denotes one specific type of detection module


\item We have $\NumClassification$ possible {\em attack classification} modules
and $\Classification_\ClassificationIndex$ with $\ClassificationIndex \in
1\dots\NumClassification$ denotes one specific type of classification module

\item We have $\NumResponse$ possible {\em attack response} modules 
 and $\Response_\ResponseIndex$ with $\ResponseIndex \in 1\dots\NumResponse$ 
denotes one specific type of response module

\item   We assume we have some pre-provisioned  total capacity  for each type
of detection, response, classification module at each location $\Pop$.  Let
$\CapacityInstances_{\Pop,\DetectionIndex}$,
$\CapacityInstances_{\Pop,\ClassificationIndex}$,
$\CapacityInstances_{\Pop,\ResponseIndex}$ respectively denote the total
provisioned capacity in terms of the {\em number of instances} of $\Pop$ for
detection module $\DetectionIndex$, classification module
$\ClassificationIndex$ and response module $\ResponseIndex$ respectively.

\item  We assume each {\em instance} (say a virtual appliance) of a particular
type  if deployed has a fixed  total   capacity;
$\CapacityPerInstance_\DetectionIndex$,
$\CapacityPerInstance_\ClassificationIndex$,
$\CapacityPerInstance_\ResponseIndex$ denotes the volume of traffic  each
instance can handle.

\item We use the generic index $\Instance$ to refer to one of these module
 instances running somewhere. $\Type_\Instance$ identifies the type of 
 the instance and $\Location_\Instance$  gives its location 


\item We assume that {\em all traffic} from  $\Traffic_{\PopA,\PopB}$ undergoes
some detection logic. The specific modules may be different.  We use indicator
values $\DetectionReqd_{\PopA,\PopB,\DetectionIndex}$ to denote if the traffic
from $\PopA$ to $\PopB$ requires the detection module $\DetectionIndex$.

%Let
%$\FootPrint_{\PopA,\PopB,\DetectionIndex}$ denote the per-traffic unit
%footprint cost of running the detection module $\DetectionIndex$ on traffic
%from $\PopA$ to $\PopB$. If some detection module is not required,
% then the footprint is simply set to zero.

\item However only the potential attack traffic undergoes the required
classification and response modules.
%  Let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ denote the cost
%of running the classification module $\ClassificationIndex$ for the potential
%attack traffic of type $\AttackIndex$ from  $\PopA$ to $\PopB$. Again this is
%zero if this type of analysis is not required.  Similarly, let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ denote the cost  of
%running the response module $\ResponseIndex$ for the potential attack traffic
%of type $\AttackIndex$ from  $\PopA$ to $\PopB$
 Similarly to the detection case, we use indicator values
$\ClassificationReqd_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ and
$\ResponseReqd_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ to denote if the
corresponding classification and response modules are required for the 
 potential attack traffic from $\PopA$ to $\PopB$.

\item There might also be a specific {\em chaining} of modules that need 
 to be applied for each $ \PopA,\PopB,\AttackIndex$ tuple. Let $\Chain_{\PopA,\PopB,\AttackIndex}$
 denote the specific chain of modules required in terms of the required classification/response 
 capabilities.   We use $|\Chain_{\PopA,\PopB,\AttackIndex}|$ to denote the length 
 of the chain, and $\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]$ to denote the module 
 function at the $\ChainLocation^\mathit{th}$ point in the chain.
 Let $\Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]}$  denote the type 
 of module at this point in the chain.
} 






==> formulation/formulation.tex <==
\section{Formulation}

\subsection{Decision variables}

\begin{itemize}

\item  We need to decide how many instances we need. We use the {\em binary decision variables} -- 
 $\ActiveInstance_{\Pop,\DetectionIndex,\Instance}, 1\dots\CapacityInstances_{\Pop,\DetectionIndex}$,
 $\ActiveInstance_{\Pop,\ClassificationIndex,\Instance},1\dots\CapacityInstances_{\Pop,\ClassificationIndex}$,
 $\ActiveInstance_{\Pop,\ResponseIndex,\Instance},1\dots\CapacityInstances_{\Pop,\ResponseIndex}$  -- to denote if we 
have activated the corresponding instance at a given $\Pop$.
  

\item  We need to decide how to {\em mirror} the traffic for the required
 monitoring and detection tasks. We  denote  the volume of traffic routed/mirrored from the ingress
to a specific instance for monitoring as $\TrafficFlow_{\PopA,\PopB,\Instance}$ 

\item  We need to decide how to {\em route} the traffic for the required
detection, classification, processing etc.  Let
$\TrafficFlow_{\AttackIndex,\PopA,\PopB,\Instance,\InstanceToo}$ denote the
volume of traffic routed for a specific potential attack traffic type from one
instance to another.    (Of course if the attack class does not require the
processing offered by the instance, these variables will never appear.)


As a special case we have $\TrafficFlow_{\PopA,\AttackIndex,\Instance}$ to denote the
 first hop from the ingress location $\PopA$ to the first instance in the 
$\Chain_{\PopA,\PopB,\AttackIndex}$. Similarly, we have a separate last-hop 
 flow $\TrafficFlow_{\AttackIndex,\Instance,\PopB}$ from a module 
 instance to the egress location $\PopB$

\end{itemize}


\subsection{Full blown optimization}


\begin{itemize}



\item Processing requirement for detection for each entering traffic to meet the required set of detection tasks 

 \begin{align}
 \forall \PopA,\PopB, \DetectionIndex \mathit{s.t.} \DetectionReqd_{\PopA,\PopB,\DetectionIndex} =1   : \sum_{\Instance: \Type_\Instance = \DetectionIndex}  \TrafficFlow_{\PopA,\PopB,\Instance}  = \Traffic_{\PopA,\PopB}  
 \end{align}


\item Processing requirement for each attack class, modeled as {\em flow conservation} equations

 \begin{align}
 \forall \PopA,\PopB, \AttackIndex, \ChainLocation, \Instance,\ \mathit{s.t.}\ \Type_\Instance = \Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]} : \nonumber \\
 \sum_{\InstanceToo: \Type_\InstanceToo = \Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation-1] }} \TrafficFlow_{\AttackIndex,\PopA,\PopB,\InstanceToo,\Instance} =  \sum_{\InstanceThree: \Type_\InstanceThree = \Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation+1] }}  \TrafficFlow_{\AttackIndex,\PopA,\PopB,\Instance,\InstanceThree} 
 \end{align}

\item there will be similar equations for the entry and exit nodes separately, where the total volume 
 has to be equal to the volume of the attack traffic

\item Model total load on each instance

 \begin{align}
 \forall \Instance: \Load_{\Pop,\ClassificationIndex,\Instance} = \sum_{\PopA,\PopB,\AttackIndex,\InstanceToo \mathit{s.t.} \exists \ChainLocation \Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]} = \Type_\Instance \& \Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation-1]} = \Type_\InstanceToo } \TrafficFlow_{\AttackIndex,\PopA,\PopB,\InstanceToo,\Instance} 
 \end{align}

\item Total load on each instance has to be less than the capacity and cannot be allowed if it is not activated 
 \begin{align}
 \forall \Pop, \DetectionIndex, \Instance: \Load_{\Pop,\DetectionIndex,\Instance} \leq \ActiveInstance_{\Pop,\DetectionIndex,\Instance} \times \CapacityPerInstance_\DetectionIndex \\ 
 \forall \Pop, \ClassificationIndex, \Instance: \Load_{\Pop,\ClassificationIndex,\Instance} \leq \ActiveInstance_{\Pop,\ClassificationIndex,\Instance} \times \CapacityPerInstance_\ClassificationIndex \\ 
 \forall \Pop, \ResponseIndex, \Instance: \Load_{\Pop,\ResponseIndex,\Instance} \leq \ActiveInstance_{\Pop,\ResponseIndex,\Instance} \times \CapacityPerInstance_\ResponseIndex  
\end{align}



\item Modeling total number of active instances: 

 \begin{equation}
 \sum_{\Pop} \sum_{\DetectionIndex} \sum_{\Instance: \Type_\Instance=\DetectionIndex,\Location_\Instance=\Pop} \ActiveInstance_{\Pop,\DetectionIndex,\Instance} +   \sum_{\Pop} \sum_{\ResponseIndex} \sum_{\Instance: \Type_\Instance=\Classification,\Location_\Instance=\Pop} \ActiveInstance_{\Pop,\ResponseIndex,\Instance} +   \sum_{\Pop} \sum_{\ClassificationIndex}  \sum_{\Instance: \Type_\Instance=\ResponseIndex,\Location_\Instance=\Pop} \ActiveInstance_{\Pop,\ClassificationIndex,\Instance}  
\end{equation}

\item Total number of instance in one location
\begin{equation}
\end{equation}

\item Total footprint, latency etc can also be modeled in terms of the $\TrafficFlow$ values


\end{itemize}


==> formulation/macros_vyas.tex <==
 
\newcommand{\TrafficClass}{\ensuremath{\mathit{class}}}
\newcommand{\TrafficClassIndex}{\ensuremath{\mathit{o}}}
\newcommand{\Traffic}{\ensuremath{\mathit{T}}}
\newcommand{\FootPrint}{\ensuremath{\mathit{F}}}
\newcommand{\Pop}{\ensuremath{\mathit{l}}}
\newcommand{\PopA}{\ensuremath{\mathit{l_\mathit{in}}}}
 \newcommand{\PopB}{\ensuremath{\mathit{l_\mathit{out}}}}
 \newcommand{\Attack}{\ensuremath{\mathit{A}}}
 \newcommand{\NumAttacks}{\ensuremath{\mathit{N}_\Attack}}
 \newcommand{\AttackIndex}{\ensuremath{\mathit{g}}}
 \newcommand{\Detection}{\ensuremath{\mathit{D}}}
 \newcommand{\NumDetection}{\ensuremath{\mathit{N}_\Detection}}
 \newcommand{\DetectionIndex}{\ensuremath{\mathit{d}}}
 \newcommand{\Classification}{\ensuremath{\mathit{C}}}
 \newcommand{\ClassificationIndex}{\ensuremath{\mathit{c}}}
 \newcommand{\NumClassification}{\ensuremath{\mathit{N}_\Classification}}
 \newcommand{\Response}{\ensuremath{\mathit{R}}}
 \newcommand{\ResponseIndex}{\ensuremath{\mathit{r}}}
 \newcommand{\NumResponse}{\ensuremath{\mathit{N}_\Response}}
 \newcommand{\CapacityInstances}{\ensuremath{\mathit{TotalInstances}}}
 \newcommand{\CapacityPerInstance}{\ensuremath{\mathit{Cap}}}
 \newcommand{\DetectionReqd}{\ensuremath{\mathit{DREQD}}}
 \newcommand{\ClassificationReqd}{\ensuremath{\mathit{CREQD}}}
 \newcommand{\ResponseReqd}{\ensuremath{\mathit{RREQD}}}
 \newcommand{\CRChain}{\ensuremath{\mathit{Chain}}}
 
 \newcommand{\ActiveInstance}{\ensuremath{\mathit{h}}}
 \newcommand{\TrafficFlow}{\ensuremath{\mathit{f}}}
 \newcommand{\Instance}{\ensuremath{\mathit{j}}}
 \newcommand{\InstanceToo}{\ensuremath{\mathit{j'}}}
 \newcommand{\InstanceThree}{\ensuremath{\mathit{j''}}}
 \newcommand{\Type}{\ensuremath{\mathit{Type}}}
 \newcommand{\Location}{\ensuremath{\mathit{Loc}}}
 \newcommand{\Load}{\ensuremath{\mathit{Load}}}
 \newcommand{\Chain}{\ensuremath{\mathit{Chain}}}
 \newcommand{\ChainLocation}{\ensuremath{\mathit{k}}}



==> formulation/requirements.tex <==
\section{System requirements}

Our goal is three-fold:

\begin{itemize}

\item Decide how many {\em instances} of each type of detection, classification, and 
 response modules we need at each location. 

\item Set up the correct routing logic so that the classification and response chain is setup 
 correctly  and that the service chain is implemented correctly

\item Objectives: 
	\begin{itemize}
	\item minimize total latency on impact, 
	\item drop attack traffic as soon as possible,
	\item minimize network congestion as much as possible, 
	\item use as few instances as possible   to minimize total operating cost
	\end{itemize}
\end{itemize}


==> formulation/seyed_centralized_and_dist/algorithms.tex <==
\section{Algorithms}

\subsection{DSP}
\begin{itemize}

\item There are many ways of assigning traffic to data centers. We want to find the solution 
that minimizes the cost.

\item We design a greedy algorithm to solve DSP with the goal of reducing ISP-wide attack footprint. 
In particular, the algorithm prioritizes higher volume attacks. Further, for given attack, it tries to assign
it to the data center that causes minimum cost. The pseudocode is outlines in the following Listing.

\item $\vms_{\attackindex,\vertexindexi}^\datacenterindex$ denotes the required number of VMs of module
type $\vertexindexi$ at data center $\datacenterindex$.

\item The output of the algorithm are:

\begin{itemize}

\item $\vms_{\attackindex,\vertexindexi}^\datacenterindex$ values (hence physical graphs)

\item $\fraction_{\edgepopindex,\attackindex,\datacenterindex}$ values

\end{itemize}

\end{itemize}

\begin{codebox}
% \li Sort $\boldsymbol{\attack}$ in increasing order of $\vms_\attackindex$ values and store the result
% in list  $\boldsymbol{\attack}'$
  
\li Build max-heap  $\boldsymbol{\Traffic}^{maxHeap}$ based on attack volumes $\boldsymbol{\Traffic}$ 
 
% \li For each edge PoP $\edgepopindex$, build a min-heap 
% $\boldsymbol{\cost^{maxHeap}_\edgepopindex}$  of cost values  
% $\cost_{\edgepopindex,\datacenterindex}$
 
 \li \While $!Empty(\boldsymbol{\Traffic}^{maxHeap})$
 
 \li \Do $\atraffic_{current} \gets ExtractMax(\boldsymbol{\Traffic}^{maxHeap})$

 \li $\datacenterindex_{current} \gets$ data center $\datacenterindex$ 
 with smallest $\cost_{\atraffic_{current}.e,\datacenterindex}$ value and non-zero capacity
 
 \li $\atraffic_1 \gets min(\atraffic_{current}, \capacity^{link}_{\datacenterindex})$
 \Comment accounting for data center link capacity
 
 \li $ \atraffic_2 \gets$ largest traffic volume $\atraffic^{max}$ such that 
 $\atraffic^{max} \leq\frac{\capacity^{Compute}_{\datacenterindex_{current}}}{\sum\limits_{\vertexindexi}{}
 \frac{\sum\limits_{\vertexindexj}{}{\weight_{\attackindex,\vertexindexj \rightarrow \vertexindexi}}}{\power_{\attackindex,\vertexindexi}}}$
 
 \li $\atraffic_{assigned} \gets min(\atraffic_1, \atraffic_2)$
 \Comment accounting for data center compute capacity
 
 
 \li $\fraction_{\edgepopindex,\attackindex,\datacenterindex} \gets 
 \frac{\atraffic_{assigned}}{\traffic_{current.\edgepopindex,current.\attackindex}}$
 
 \li \For each module type \vertexindexi
 \li \Do 
 
\li  $\vms_{\attackindex,\vertexindexi}^\datacenterindex = 
\vms_{\attackindex,\vertexindexi}^\datacenterindex +
 \atraffic_{assigned}^\datacenterindex 
 \times 
 {
 \frac{\sum\limits_{\vertexindexj}{}{\weight_{\attackindex,\vertexindexj \rightarrow \vertexindexi}}}{\power_{\attackindex,\vertexindexi}}}$ \Comment update  number of modules of type 
 $\vertexindexi$ at data center $\datacenterindex$

\End

 \li $\capacity^{link}_{\datacenterindex_{current}} \gets \capacity^{link}_{\datacenterindex_{current}} -  \atraffic_{assigned} $ \Comment update data center's link capacity

 \li $\capacity^{compute}_{\datacenterindex_{current}} \gets 
 \capacity^{compute}_{\datacenterindex_{current}} -  \atraffic_{assigned} 
 \times 
 {\sum\limits_{\vertexindexi}{}
 \frac{\sum\limits_{\vertexindexj}{}{\weight_{\attackindex,\vertexindexj \rightarrow \vertexindexi}}}{\power_{\attackindex,\vertexindexi}}}$ \Comment update data center's compute capacity
 
 \li $\atraffic_{unassigned} = \atraffic_{current} - \atraffic_{assigned}$
 
 \li \If ($\atraffic_{unassigned} > 0$) 
 
 \li 		\Then
 
 \li $InsertElement(\boldsymbol{\Traffic}^{maxHeap}, \atraffic_{unassigned})$
\End

 \End
 

\comment{ 
\li  \For $\attackindex' \gets 1$ to $\mid \boldsymbol{\attack} \mid$
\li \Do  \For $l' \gets 1$ to $\mid \boldsymbol{\cost'} \mid$	
\li \Do $\edgepopindex'  \gets \edgepopindex$ where $\boldsymbol{\cost}'[l']$ = $\cost_{\edgepopindex,\datacenterindex}$
\li $\datacenterindex'  \gets \datacenterindex$ where $\boldsymbol{\cost}'[l']$ = $\cost_{\edgepopindex,\datacenterindex}$
\li Assign as much of traffic $\Traffic_{\edgepopindex',\attackindex'}$ as possible to
data center $\datacenter_{\datacenterindex'}$
\li Update $\Traffic_{\edgepopindex',\attackindex'}$, $\capacity^{link}_{\datacenterindex'}$, and
$\capacity^{compute}_{\datacenterindex'}$ values as per the assignment
\li Terminate if all traffic is assigned or no assignment is possible
\End
\End
}
\end{codebox}


\subsection{SSP}

\begin{itemize}

\item explain stuff

\end{itemize}

\begin{codebox}

\li \For each data center $\datacenterindex$

\li \Do Sort aggregate places in decreasing order of available VM slots

\li In each aggregate place, sort racks in decreasing order of available VM slots

\li In each rack, sort servers in decreasing order of available VM slots

\li \For each physical graph $\graph^{\physical}_\attackindex=(\vertexes^{\physical}_\attackindex,\edges^{\physical}_\attackindex)$ located in $\datacenterindex$

%\li \Do \While ($\graph^{\physical}_\attackindex$ is not assigned)
\li \Do Try to assign the entire $\graph^{\physical}_\attackindex$ to the server with largest open slots
\li \If failed 
\li \Then Try to assign the entire $\graph^{\physical}_\attackindex$ to the rack with largest open slots
\li \If failed
\li \Then Try to assign the entire $\graph^{\physical}_\attackindex$ to the agg. place with largest open slots
\li \If failed
\li \Then Do any arbitrary assignment
\End
\End

\End

\end{codebox}

{\bf Discussion/eval point} how to realize  graphs in data centers? extreme 1: one giant graph 
(resulted by scaling) of each logical graph, extreme 2: no scaling, simply replicate the whole 
logical graph as needed.

\subsection{Centralized Algorithm}
In this subsection we show the joint optimization of DSP and SSP sung an ILP formulation.
In addition to parameters and variables that we have defined earlier, we define the binary
variable $\vmassigned_{\attackindex,\vertexindexi,\vmindex,\datacenterindex,\arack,\aserver}$ 
as follows: if  it is 1, it 
means VM $\vmindex$ of type $\vertex_{\attackindex,\vertexindexi}$ runs on  server $\aserver$ of
rack $\arack$; otherwise, 
$\vmassigned_{\attackindex,\vertexindexi,\vmindex,\datacenterindex,\arack,\aserver}=0$. Each unit
of intra- and inter cross-rack traffic costs $\unitIntraRackCost$ and $\unitInterRackCost$ 
(e.g., represent latency).

%ILP
\begin{codebox}
%objective function
\li minimize
$\sum\limits_{\edgepopindex}^{}
\sum\limits_{\attackindex}^{}
\sum\limits_{\datacenterindex}^{}
\fraction_{\edgepopindex,\attackindex,\datacenterindex}
\times
\Traffic_{\edgepopindex,\attackindex}
\times
\cost_{\edgepopindex,\datacenterindex}
+
\sum\limits_{\datacenterindex}^{}
\datacentercost_{\datacenterindex}
$

\li s.t.

%all attack being dealt with
\li $ \forall  \edgepopindex, \attackindex:
\sum\limits_{\datacenterindex}^{}
\fraction_{\edgepopindex,\attackindex,\datacenterindex} = 1$\Comment all attack traffic should be served

%total data center traffic
\li $ \forall \attackindex, \datacenterindex:
\atraffic_{\attackindex, \datacenterindex}
=
\sum\limits_{\edgepopindex}^{}
\fraction_{\edgepopindex,\attackindex,\datacenterindex}
\times
\Traffic_{\edgepopindex,\attackindex}$ \Comment total traffic volume going to each data center

%data center link capacity
\li $ \forall \datacenterindex:
\sum\limits_{\attackindex}\atraffic_{\attackindex, \datacenterindex}
\leq
\capacity^{link}_{\datacenterindex}$ \Comment data center link capacity

%getting enough vms of each module
\li $ \forall \datacenterindex, \attackindex, \vertexindexi:
\vms_{\attackindex,\vertexindexi}^\datacenterindex 
\geq
\atraffic_{\attackindex, \datacenterindex} 
\times
\frac{\sum\limits_{\vertexindexj}{}{\weight_{\attackindex,\vertexindexj \rightarrow \vertexindexi}}}{\power_{\attackindex,\vertexindexi}}$ \Comment provisioning sufficient VMs of each module type

%data center compute capacity
\li $\forall \datacenterindex:
\sum\limits_{\attackindex}
\sum\limits_{\vertexindexi}
\vms_{\attackindex,\vertexindexi}^\datacenterindex 
\leq
\capacity^{compute}_{\datacenterindex}$ \Comment data center compute capacity

%bandwidth cost
\li $ \forall \datacenterindex:
\datacentercost_\datacenterindex: = \interrack_\datacenterindex + \intrarack_\datacenterindex
$

%intra-rack traffic cost factor
\li $ \forall \datacenterindex:
\intrarack_{\datacenterindex}
=
\sum\limits_{\edge_{\attackindex,\vertexindexi \rightarrow \vertexindexj}^{\logical} 
\in \graph^{\logical}_\attackindex 
\wedge
(\vertexindexi , \vertexindexj) \notin sameServer
\wedge
(\vertexindexi , \vertexindexj) \in sameRack}
\vmassigned_{\attackindex,\vertexindexi,\vmindex,\datacenterindex, \arack,\aserver}
\times
\weight_{\attackindex,\vertexindexj \rightarrow \vertexindexi}
\times \unitInterRackCost
$\Comment inter rack cost

%inter-rack traffic cost factor
\li $ \forall \datacenterindex:
\interrack_{\datacenterindex}
=
\sum\limits_{\edge_{\attackindex,\vertexindexi \rightarrow \vertexindexj}^{\logical} 
\in \graph^{\logical}_\attackindex 
\wedge
(\vertexindexi , \vertexindexj) \notin sameRack}
\vmassigned_{\attackindex,\vmindex,\vertexindexi,\datacenterindex, \arack,\aserver}
\times
\weight_{\attackindex,\vertexindexj \rightarrow \vertexindexi}
\times \unitInterRackCost
$\Comment inter rack cost

%counting modules
\li $ \forall \datacenterindex, \attackindex, \vertexindexi:
\vms_{\attackindex,\vertexindexi}^\datacenterindex 
=
\sum\limits_{\servers \in \datacenterindex}
\sum\limits_{\racks \in \datacenterindex}
\vmassigned_{\attackindex,\vertexindexi,\vmindex,\datacenterindex, \arack,\aserver}
$ \Comment counting VMs of each module type

%decision variables
\li decision variables: 
$\fraction_{\edgepopindex,\attackindex,\datacenterindex} \in [0,1],
\vmassigned_{\attackindex,\vertexindexi,\vmindex,\datacenterindex, \arack,\aserver} \in \{0,1\},
\vms_{\attackindex,\vertexindexi}^\datacenterindex \in \{0,1,\dots\},
\interrack_{\datacenterindex}, \atraffic_{\attackindex, \datacenterindex} \in \mathbb{R}
$

\end{codebox}













==> formulation/seyed_centralized_and_dist/analysis.tex <==
\section{Analysis and Discussion}


==> formulation/seyed_centralized_and_dist/macros_dist.tex <==
\newcommand{\edgepopindex}{\ensuremath{\mathit{e}}}
\newcommand{\edgepop}{\ensuremath{\mathit{E}}}
\newcommand{\attackindex}{\ensuremath{\mathit{a}}}
\newcommand{\attack}{\ensuremath{\mathit{A}}}
\newcommand{\datacenterindex}{\ensuremath{\mathit{d}}}
\newcommand{\datacenter}{\ensuremath{\mathit{D}}}
\newcommand{\traffic}{\ensuremath{\mathit{T}}}
\newcommand{\atraffic}{\ensuremath{\mathit{t}}}
\newcommand{\vms}{\ensuremath{\mathit{N}}}
\newcommand{\capacity}{\ensuremath{\mathit{C}}}
\newcommand{\cost}{\ensuremath{\mathit{L}}}
\newcommand{\fraction}{\ensuremath{\mathit{f}}}


\newcommand{\graph}{\ensuremath{\mathit{G}}}
\newcommand{\vertexes}{\ensuremath{\mathit{V}}}
\newcommand{\vertex}{\ensuremath{\mathit{v}}}
\newcommand{\vertexindexi}{\ensuremath{\mathit{i}}}
\newcommand{\vertexindexj}{\ensuremath{\mathit{j}}}
\newcommand{\edges}{\ensuremath{\mathit{E}}}
\newcommand{\edge}{\ensuremath{\mathit{e}}}
\newcommand{\weight}{\ensuremath{\mathit{w}}}
\newcommand{\logical}{\ensuremath{\mathit{logical}}}
\newcommand{\physical}{\ensuremath{\mathit{physical}}}
\newcommand{\power}{\ensuremath{\mathit{P}}}

\newcommand{\vmassigned}{\ensuremath{\mathit{q}}}
\newcommand{\vmindex}{\ensuremath{\mathit{v}}}
\newcommand{\servers}{\ensuremath{\mathit{Servers}}}
\newcommand{\aserver}{\ensuremath{\mathit{s}}}
%\newcommand{\slots}{\ensuremath{\mathit{Slots}}}
%\newcommand{\aslot}{\ensuremath{\mathit{slot}}}
\newcommand{\racks}{\ensuremath{\mathit{Racks}}}
\newcommand{\arack}{\ensuremath{\mathit{r}}}
\newcommand{\unitIntraRackCost}{\ensuremath{\mathit{Intra}}}
\newcommand{\unitInterRackCost}{\ensuremath{\mathit{Inter}}}
\newcommand{\datacentercost}{\ensuremath{\mathit{DSC}}}
\newcommand{\interrack}{\ensuremath{\mathit{InterRack}}}
\newcommand{\intrarack}{\ensuremath{\mathit{IntraRack}}}

%%%%%%%%%OLD STUFF%%%%%%%%%%%
%\comment{ 
\newcommand{\Traffic}{\ensuremath{\mathit{T}}}
\newcommand{\FootPrint}{\ensuremath{\mathit{F}}}
\newcommand{\Pop}{\ensuremath{\mathit{l}}}
\newcommand{\PopA}{\ensuremath{\mathit{l_\mathit{in}}}}
 \newcommand{\PopB}{\ensuremath{\mathit{l_\mathit{out}}}}
 \newcommand{\Attack}{\ensuremath{\mathit{A}}}
 \newcommand{\NumAttacks}{\ensuremath{\mathit{N}_\Attack}}
 \newcommand{\AttackIndex}{\ensuremath{\mathit{j}}}
 \newcommand{\Detection}{\ensuremath{\mathit{D}}}
 \newcommand{\NumDetection}{\ensuremath{\mathit{N}_\Detection}}
 \newcommand{\DetectionIndex}{\ensuremath{\mathit{d}}}
 \newcommand{\Classification}{\ensuremath{\mathit{C}}}
 \newcommand{\ClassificationIndex}{\ensuremath{\mathit{c}}}
 \newcommand{\NumClassification}{\ensuremath{\mathit{N}_\Classification}}
 \newcommand{\Response}{\ensuremath{\mathit{R}}}
 \newcommand{\ResponseIndex}{\ensuremath{\mathit{r}}}
 \newcommand{\NumResponse}{\ensuremath{\mathit{N}_\Response}}
 \newcommand{\CapacityInstances}{\ensuremath{\mathit{TotalInstances}}}
 \newcommand{\CapacityPerInstance}{\ensuremath{\mathit{Cap}}}
 \newcommand{\DetectionReqd}{\ensuremath{\mathit{DREQD}}}
 \newcommand{\ClassificationReqd}{\ensuremath{\mathit{CREQD}}}
 \newcommand{\ResponseReqd}{\ensuremath{\mathit{RREQD}}}
 \newcommand{\CRChain}{\ensuremath{\mathit{Chain}}}
 
 \newcommand{\ActiveInstance}{\ensuremath{\mathit{d}}}
 \newcommand{\TrafficFlow}{\ensuremath{\mathit{f}}}
 \newcommand{\Instance}{\ensuremath{\mathit{j}}}
 \newcommand{\InstanceToo}{\ensuremath{\mathit{j'}}}
 \newcommand{\InstanceThree}{\ensuremath{\mathit{j''}}}
 \newcommand{\Type}{\ensuremath{\mathit{Type}}}
 \newcommand{\Location}{\ensuremath{\mathit{Loc}}}
 \newcommand{\Load}{\ensuremath{\mathit{Load}}}
 \newcommand{\Chain}{\ensuremath{\mathit{Chain}}}
 \newcommand{\ChainLocation}{\ensuremath{\mathit{k}}}
%}

==> formulation/seyed_centralized_and_dist/requirements.tex <==
\section{System requirements}

Our goal is three-fold:

\begin{itemize}

\item Decide how many {\em instances} of each type of detection, classification, and 
 response modules we need at each location. 

\item Set up the correct routing logic so that the classification and response chain is setup 
 correctly  and that the service chain is implemented correctly

\item Objectives: 
	\begin{itemize}
	\item minimize total latency on impact, 
	\item drop attack traffic as soon as possible,
	\item minimize network congestion as much as possible, 
	\item use as few instances as possible   to minimize total operating cost
	\end{itemize}
\end{itemize}


==> formulation/seyed_centralized_and_dist/system.tex <==
\section{Problem Definition}

\subsection{Setup}

\begin{itemize}

\item {\bf Note 1:} For clarity, what we present here is with respect to one particular customer 
(it is trivial to extend it to the case of multiple customers).

\item {\bf Note 2:} We assume C (classification) is already completed, so now we are
able to distinguish suspicious traffic at the ingress.

\item {\bf Note 3:} We focus on the task of resource assignment to determine how many VMs and
where (i.e., which data centers and which servers inside the selected data centers) to launch
as to implement the required A (analysis) and R (response).

\item {\bf Logical graphs:} There are different types DDoS
 attacks which naturally require different
analyses and responses. A logical graph 
$\graph^{\logical}_\attackindex=(\vertexes^{\logical}_\attackindex,\edges^{\logical}_\attackindex)$ 
is a weighted DAG that represents the logical interconnection of analysis and response modules that
traffic of attack type  $\attackindex$ needs to go through. The ISP operator populates a library of
such logical graphs, one per attack type.
Figure~\ref{fig:logical_graph} shows an example logical graph that we use for SYN flood
attacks with 
$\mid \vertexes^{\logical}_\attackindex \mid = 6$ 
and 
$\mid \edges^{\logical}_\attackindex \mid = 5$. Let 
$\vertex_{\attackindex,\vertexindexi}^{\logical}$ 
denote vertex $\vertexindexi$ of $\graph^{\logical}_\attackindex$, and
$\edge_{\attackindex,\vertexindexi \rightarrow \vertexindexj}^{\logical}$ 
denote the edge from vertex $\vertex_{\attackindex,\vertexindexi}^{\logical}$
to vertex $\vertex_{\attackindex,\vertexindexj}^{\logical}$.
 The weight of
$\edge_{\attackindex,\vertexindexi \rightarrow \vertexindexj}^{\logical}$
is denoted by
$\weight_{\attackindex,\vertexindexi \rightarrow \vertexindexj}$, which represents
what fraction of the total graph input traffic is expected to traverse 
$\edge_{\attackindex,\vertexindexi \rightarrow \vertexindexj}^{\logical}$\footnote{These
weights are computed based on past data.}. For example, in Figure~\ref{fig:logical_graph},
$\weight_{synflood,{hids} \rightarrow {logging}} = 0.25$ means a quarter of the input
traffic to the graph is expected to be sent to the logging module by the heavy IPS (H-IDS) 
module.

\begin{figure}[h]
\centering
\includegraphics[width=340pt]{figs/logical_graph.pdf}
\tightcaption{An example logical graph for SYN flood.}
\label{fig:logical_graph}
\end{figure}

\item {\bf Physical graphs:} A physical graph 
$\graph^{\physical}_\attackindex=(\vertexes^{\physical}_\attackindex,\edges^{\physical}_\attackindex)$ 
is a physical realization of logical graph $\graph^{\logical}_\attackindex$: each node of 
$\graph^{\logical}_\attackindex$ will be realized via one or multiple nodes of 
$\graph^{\physical}_\attackindex$ depending on the input traffic volume.
To determine how many physical nodes (i.e., VMs) are required to realize 
$\vertex_{\attackindex,\vertexindexi}^{\logical}$,
we need to consider the traffic processing capacity of each VM of type 
$\vertex_{\attackindex,\vertexindexi}^{\logical}$. To put this in context, note that
everything else being equal, the processing capacity of a VM depends on the nature
of traffic processing that it performs, which is attack-dependent. 
Going back to the example of Figure~\ref{fig:logical_graph},  if each L-IDS VM  has a 
capacity of processing at most 1Gbps of attack traffic, and if the input traffic is 3Gbps 
in a particular network, L-IDS should be realized via 3 physical nodes (i.e., VMs).
$\power_{\attackindex,\vertexindexi}$ denotes the traffic processing capacity of a VM
of type $\vertexes^{\physical}_\attackindex$ (e.g., it is 1Gbps in this example for a L-IDS
in this example).

\item {\bf ISP architecture:} As shown in Figure~\ref{fig:isp}, the ISP is composed of  a set of edge PoPs 
$\boldsymbol{\edgepop}=
\{\edgepop_1,\dots, \edgepop_{\edgepopindex},\dots, \edgepop_{\mid \boldsymbol{\edgepop} \mid}\}$, 
a set of data centers 
$\boldsymbol{\datacenter}=
\{\datacenter_1,\dots, \datacenter_{\datacenterindex},\dots, \datacenter_{\mid \boldsymbol{\datacenter} \mid}\}$, 
a global controller, and high-capacity backbone switches and links\footnote{We assume 
backbone switches and links do not cause congestion.}. The high-level role of the ISP is 
to transit traffic between its edge PoPs.

\begin{figure}[h]
\centering
\includegraphics[width=340pt]{figs/zoomout_view.pdf}
\tightcaption{ISP architecture.}
\label{fig:isp}
\end{figure}

\item {\bf Data center architecture:} Zooming into a data center $\datacenter_{\datacenterindex}$ 
shown in Figure~\ref{fig:data_center}, it is assumed to have a typical hierarchical topology of 
switches. 

\begin{figure}[h]
\centering
\includegraphics[width=280pt]{figs/zoomin_view.pdf}
\tightcaption{Data center architecture.}
\label{fig:data_center}
\end{figure}

\item The goal of the {\bf resource assignment problem} is to decide which servers are responsible 
for processing (i.e., running the required A and R modules) for the ISP-wide input attack traffic.

\item {\bf Challenges of a centralized solutions} The ILP formulation gives a globally optimal solution 
to the resource assignment problem. However, it is hindered by two serious problems: scalability and 
centrality. Besides being too slow, it is not practical to maintain all low-level (e.g., a VM swap 
out event on a server) in a centralized manner. We, therefore, aim to provide a natural distributed 
solution to this problem.

\item {\bf Distributed approach} We decompose the resource assignment problem into two natural
sub-problems:

{\bf (1) Data Center Selection Problem (DSP)}: Assigning input attack traffic to data centers.

{\bf (2) Server Selection Problem (SSP)}: Assigning servers inside each selected data center
(as given by DSP) to run the required A and R modules to process the assigned attack traffic.

\end{itemize}


\subsection{Data Center Selection Problem (DSP)}

\begin{itemize}

\item  {\bf Notations:} Let  $\boldsymbol{\attack}=
\{\attack_1,\dots, \attack_{\attackindex},\dots, \attack_{\mid \boldsymbol{\attack} \mid}\}$
denote the set of possible DDoS attacks (e.g., SYN flood, NTP amplification).  
Further, let $\Traffic_{\edgepopindex,\attackindex}$ 
denote the total volume of attack traffic of type $\attackindex \in \boldsymbol{\attack}$ 
 at ingress $\edgepopindex \in \boldsymbol{\edgepop}$ destined to the customer. 
Let 
$\mid \boldsymbol{\Traffic} \mid = 
\{
\Traffic_{1,1},
\dots,
\Traffic_{\edgepopindex,\attackindex},
\dots,
\Traffic_{\mid \boldsymbol{\edgepop}\mid ,\mid \boldsymbol{\attack}\mid },
\}$
denote the set of all attack traffic volumes.
 
Note that $\Traffic_{\edgepopindex,\attackindex}$ requires to be ``dealt with''; (i.e., 
it needs to go through the required sequence of A and R modules at some data 
center(s).\footnote{Non-attack traffic is simply forwarded to the customer after 
traversing backbone links and switches (without going to any data center).} The cost 
of transferring each unit of traffic from ingress $\edgepopindex$ to data center 
$\datacenterindex$ is $\cost_{\edgepopindex,\datacenterindex}$. This cost represents 
the traffic footprint and latency associated with unit traffic.


\item {\bf Resource Constraints:} As stated before, we assume backbone links and switches 
do not cause bottleneck. However, a data center has limited link and compute capacity to 
assign to traffic. The traffic processing service that each data center
$\datacenter_\datacenterindex$ can provide is limited by two types of constraints: its current 
I/O link capacity (i.e., how much traffic the data center can transfer with the outside world) 
and its current computing capacity (i.e., what is the total available of compute capacity of its servers),
denoted by $\capacity^{link}_{\datacenterindex}$  and $\capacity^{compute}_{\datacenterindex}$,
respectively.  
%Each unit of traffic $\Traffic_{\edgepopindex,\attackindex}$ requires $\vms_\attackindex$
%VMs (to implement the required A and R modules for attack type $\attackindex$).

\item A {\bf solution} to DSP involves: 

(1) A feasible assignment of attack traffics to data centers (i.e., selected data centers have 
enough link and compute capacity to deal the assigned traffic);

(2) A feasible assignment of servers inside selected data centers to run the required VMs to 
realize the required A and R modules for the incoming attack traffic. 

Note that input traffic volume $\Traffic_{\edgepopindex,\attackindex}$ can be split
and sent to different data centers. Let $\fraction_{\edgepopindex,\attackindex,\datacenterindex}$
show the fraction of traffic $\Traffic_{\edgepopindex,\attackindex}$ that a solutions decides to
send to data center $\datacenter_\datacenterindex$. 

\item The {\bf cost of a solution} is 
$\sum\limits_{\edgepopindex=1}^{\boldsymbol{\edgepop}} 
\sum\limits_{\attackindex=1}^{\boldsymbol{\attack}}
\sum\limits_{\datacenterindex=1}^{\boldsymbol{\datacenter}}
\fraction_{\edgepopindex,\attackindex,\datacenterindex}
\Traffic_{\edgepopindex,\attackindex}
\cost_{\edgepopindex,\datacenterindex} $

\item The {\bf  optimal solution to DSP} is the solution with the lowest 
cost.\footnote{For ease of presentation, here we focus on the common 
case where the ISP has enough resources to handle the entire input attack
traffic. We generalize this in~\ref{}.}


\end{itemize}



\subsection{Server Selection Problem (SSP)}
\label{subsec:ssp_def}

\begin{itemize}

\item Inside data center $\datacenter_{\datacenterindex}$, the total current compute capacity 
$\capacity^{compute}_{\datacenterindex}$ is composed of the sum of individual compute
capacities of its servers.

\item The {\bf goal of a solution to SSP:} is to localize the VMs that implement A and R of 
a given attack as much as possible. The following four possible choices at sorted in the 
order of decreasing locality: on the same server, under the same ToR switch, under the same 
aggregate switch, and under the same core switch.

\end{itemize}

%%%%%%%%%%%%%%%%OLD STUFF BELOW%%%%%%%%%%%%%%%%
\comment{
\item We have $\NumAttacks$ possible DDoS attacks; $\Attack_\AttackIndex$ with
$\AttackIndex = 1\dots\NumAttacks$   denotes a specific type of attack.  Let
$\Traffic_{\PopA,\PopB,\AttackIndex}$ denote the total volume of {\em potential
attack} traffic of type $\AttackIndex$ from ingress $\PopA$ to egress $\PopB$.
We say potential because we may not know how much of it will be true attack
until after the required classification modules have been applied.  These are
assumed to be non-overlapping; e.g.,  things like syn-flood, NTP reflector, DNS
amplifiction, or unknown.


\item We have $\NumDetection$ possible {\em attack detection} modules and
$\Detection_\DetectionIndex$ with $\DetectionIndex \in 1\dots\NumDetection$
denotes one specific type of detection module


\item We have $\NumClassification$ possible {\em attack classification} modules
and $\Classification_\ClassificationIndex$ with $\ClassificationIndex \in
1\dots\NumClassification$ denotes one specific type of classification module

\item We have $\NumResponse$ possible {\em attack response} modules 
 and $\Response_\ResponseIndex$ with $\ResponseIndex \in 1\dots\NumResponse$ 
denotes one specific type of response module

\item   We assume we have some pre-provisioned  total capacity  for each type
of detection, response, classification module at each location $\Pop$.  Let
$\CapacityInstances_{\Pop,\DetectionIndex}$,
$\CapacityInstances_{\Pop,\ClassificationIndex}$,
$\CapacityInstances_{\Pop,\ResponseIndex}$ respectively denote the total
provisioned capacity in terms of the {\em number of instances} of $\Pop$ for
detection module $\DetectionIndex$, classification module
$\ClassificationIndex$ and response module $\ResponseIndex$ respectively.

\item  We assume each {\em instance} (say a virtual appliance) of a particular
type  if deployed has a fixed  total   capacity;
$\CapacityPerInstance_\DetectionIndex$,
$\CapacityPerInstance_\ClassificationIndex$,
$\CapacityPerInstance_\ResponseIndex$ denotes the volume of traffic  each
instance can handle.

\item We use the generic index $\Instance$ to refer to one of these module
 instances running somewhere. $\Type_\Instance$ identifies the type of 
 the instance and $\Location_\Instance$  gives its location 


\item We assume that {\em all traffic} from  $\Traffic_{\PopA,\PopB}$ undergoes
some detection logic. The specific modules may be different.  We use indicator
values $\DetectionReqd_{\PopA,\PopB,\DetectionIndex}$ to denote if the traffic
from $\PopA$ to $\PopB$ requires the detection module $\DetectionIndex$.

%Let
%$\FootPrint_{\PopA,\PopB,\DetectionIndex}$ denote the per-traffic unit
%footprint cost of running the detection module $\DetectionIndex$ on traffic
%from $\PopA$ to $\PopB$. If some detection module is not required,
% then the footprint is simply set to zero.

\item However only the potential attack traffic undergoes the required
classification and response modules.
%  Let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ denote the cost
%of running the classification module $\ClassificationIndex$ for the potential
%attack traffic of type $\AttackIndex$ from  $\PopA$ to $\PopB$. Again this is
%zero if this type of analysis is not required.  Similarly, let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ denote the cost  of
%running the response module $\ResponseIndex$ for the potential attack traffic
%of type $\AttackIndex$ from  $\PopA$ to $\PopB$
 Similarly to the detection case, we use indicator values
$\ClassificationReqd_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ and
$\ResponseReqd_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ to denote if the
corresponding classification and response modules are required for the 
 potential attack traffic from $\PopA$ to $\PopB$.

\item There might also be a specific {\em chaining} of modules that need 
 to be applied for each $ \PopA,\PopB,\AttackIndex$ tuple. Let $\Chain_{\PopA,\PopB,\AttackIndex}$
 denote the specific chain of modules required in terms of the required classification/response 
 capabilities.   We use $|\Chain_{\PopA,\PopB,\AttackIndex}|$ to denote the length 
 of the chain, and $\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]$ to denote the module 
 function at the $\ChainLocation^\mathit{th}$ point in the chain.
 Let $\Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]}$  denote the type 
 of module at this point in the chain.
} 






==> formulation/simplified/formulation.tex <==
\section{Formulation}

\subsection{Decision variables}

\begin{itemize}

\item  We need to decide how many instances we need of each type.  We use  {\em
binary decision variables} -- $\ActiveInstance_{\Instance,\DetectionIndex}$
$\ActiveInstance_{\Instance,\ClassificationIndex}$ and
$\ActiveInstance_{\Instance,\ResponseIndex}$ to denote the decision if we have
a) activated the instance and b) if it has been assigned to one of these roles.
  

\item  We need to decide how to {\em mirror} the traffic for the required
monitoring and detection tasks. We  denote  the volume of traffic
routed/mirrored from the ingress to a specific instance for monitoring as
$\TrafficFlow_{\PopA,\PopB,\Instance}$ 

\item  We need to decide how to {\em route} the traffic for the required
detection, classification, processing etc.  Let
$\TrafficFlow_{\TrafficClassIndex,\Instance,\InstanceToo,\ChainLocation}$ denote the
volume of traffic routed for a specific traffic class at the 
 chain location $\ChainLocation$ from one instance to another.    (If the class does not require the
processing offered by the instance, these variables will never appear.)


As a special case we have $\TrafficFlow_{\TrafficClassIndex,\PopA,\Instance}$ to denote the
 first hop from the ingress location $\PopA$ to the first instance in the 
$\Chain_{\TrafficClassIndex}$. Similarly, we have a separate last-hop 
 flow $\TrafficFlow_{\TrafficClassIndex,\Instance,\PopB}$ from a module 
 instance to the egress location $\PopB$

\end{itemize}


\subsection{Full blown optimization}


\begin{itemize}


\item Each instance can serve {\em at most} one role (the instance is allowed to be inactive and none of the values will be 1)

 \begin{align}
\forall \Instance:  \sum_{\DetectionIndex} \ActiveInstance_{\Instance,\DetectionIndex} + \sum_{\ClassificationIndex} \ActiveInstance_{\Instance,\ClassificationIndex} + \sum_{\ResponseIndex} \ActiveInstance_{\Instance,\ResponseIndex} \leq 1 
 \end{align}



\item Processing requirement for detection for each entering traffic to meet the required set of detection tasks 

 \begin{align}
 \forall \PopA,\PopB, \DetectionIndex\ \mathit{such\ that}\ \DetectionReqd_{\PopA,\PopB,\DetectionIndex} =1   : \sum_{\Instance}  \TrafficFlow_{\PopA,\PopB,\Instance}  = \Traffic_{\PopA,\PopB}  
 \end{align}

This traffic can be sent only if the instance has been assigned the detection role. Thus, we have:

\begin{align}
 \forall \PopA,\PopB, \Instance:   \TrafficFlow_{\PopA,\PopB,\Instance}  \leq \Traffic_{\PopA,\PopB}   \times \ActiveInstance_{\Instance,\DetectionIndex}
 \end{align}



\item Processing requirement for each attack class, modeled as {\em flow conservation} equations

 \begin{align}
 \forall \TrafficClassIndex, \Instance, \ChainLocation:  \sum_{\InstanceToo} \TrafficFlow_{\TrafficClassIndex,\InstanceToo,\Instance,\ChainLocation-1} =  \sum_{\InstanceThree}  \TrafficFlow_{\TrafficClassIndex,\Instance,\InstanceThree,\ChainLocation+1} 
 \end{align}

These flow values can only be allowed if the instances constituting the flow variable have been allocated this specific roles:

 \begin{align}
  \forall \TrafficClassIndex, \Instance, \InstanceToo, \ChainLocation:   \TrafficFlow_{\TrafficClassIndex,\InstanceToo,\Instance,\ChainLocation-1} \leq \Traffic_{\TrafficClassIndex} \times \ActiveInstance_{\Instance,\Type_{\Chain_{\TrafficClassIndex}[\ChainLocation]}}  \\
  \forall \TrafficClassIndex, \Instance, \InstanceToo, \ChainLocation:   \TrafficFlow_{\TrafficClassIndex,\InstanceToo,\Instance,\ChainLocation-1} \leq \Traffic_{\TrafficClassIndex} \times \ActiveInstance_{\InstanceToo,\Type_{\Chain_{\TrafficClassIndex}[\ChainLocation-]}}   \\
  \forall \TrafficClassIndex, \Instance, \InstanceThree, \ChainLocation:   \TrafficFlow_{\TrafficClassIndex,\Instance,\InstanceThree,\ChainLocation+1} \leq \Traffic_{\TrafficClassIndex} \times \ActiveInstance_{\Instance,\Type_{\Chain_{\TrafficClassIndex}[\ChainLocation]}}  \\
  \forall \TrafficClassIndex, \Instance, \InstanceThree, \ChainLocation:   \TrafficFlow_{\TrafficClassIndex,\Instance,\InstanceThree,\ChainLocation+1} \leq \Traffic_{\TrafficClassIndex} \times \ActiveInstance_{\InstanceThree,\Type_{\Chain_{\TrafficClassIndex}[\ChainLocation+1]}}  
 \end{align}



\item there will be similar equations for the entry and exit nodes separately, where the total volume 
 has to be equal to the volume of the attack traffic

 \begin{align}
 \forall \TrafficClassIndex:  \sum_{\Instance} \TrafficFlow_{\TrafficClassIndex,\PopA,\Instance} =  \Traffic_{\TrafficClassIndex}
 \end{align}

\begin{align}
 \forall \TrafficClassIndex:  \sum_{\Instance} \TrafficFlow_{\TrafficClassIndex,\Instance,\PopB} =  \Traffic_{\TrafficClassIndex}
 \end{align}


Again, these special flow values can only be allowed if the instances are assigned the roles of the zeroth and last location in the chain: 

 \begin{align}
  \forall \TrafficClassIndex, \Instance:   \TrafficFlow_{\TrafficClassIndex,\PopA,\Instance} \leq \Traffic_{\TrafficClassIndex} \times \ActiveInstance_{\Instance,\Type_{\Chain_{\TrafficClassIndex}[1]}}  \\
  \forall \TrafficClassIndex, \Instance:   \TrafficFlow_{\TrafficClassIndex,\Instance,\PopB} \leq \Traffic_{\TrafficClassIndex} \times \ActiveInstance_{\Instance,\Type_{\Chain_{\TrafficClassIndex}[|\Chain_{\TrafficClassIndex}|]}}
 \end{align}



\item Model total load on each instance

 \begin{align}
 \forall \Instance: \Load_{\Instance} = \sum_{\TrafficClassIndex,\ChainLocation,\InstanceToo} \TrafficFlow_{\TrafficClassIndex,\InstanceToo,\Instance,\ChainLocation}  +  \sum_{\PopA,\PopB} \TrafficFlow_{\PopA,\PopB,\Instance}
 \end{align}

\item Total load on each instance has to be less than the capacity (for a specific role) and cannot be allowed if it is not activated 
 \begin{align}
 \forall  \Instance: \Load_{\Instance} \leq  \sum_{\DetectionIndex} \ActiveInstance_{\Instance,\DetectionIndex} \CapacityPerInstance_\DetectionIndex +    \sum_{\ResponseIndex} \ActiveInstance_{\Instance,\ResponseIndex} \CapacityPerInstance_\ResponseIndex +    \sum_{\ClassificationIndex}  \ActiveInstance_{\Instance,\ClassificationIndex}   \CapacityPerInstance_\ClassificationIndex
\end{align}


\item Modeling total number of active instances: 

 \begin{equation}
 \sum_{\Instance,\DetectionIndex} \ActiveInstance_{\Instance,\DetectionIndex} +    \sum_{\Instance,\ResponseIndex} \ActiveInstance_{\Instance,\ResponseIndex} +    \sum_{\Instance,\ClassificationIndex}  \ActiveInstance_{\Instance,\ClassificationIndex}  
\end{equation}

\item Total number of instance at one location

\begin{equation}
\forall \Instance,\Pop\ \mathit{such\ that}\ \Location_\Instance = \Pop: \sum_{\Instance,\DetectionIndex} \ActiveInstance_{\Instance,\DetectionIndex} +    \sum_{\Instance,\ResponseIndex} \ActiveInstance_{\Instance,\ResponseIndex} +    \sum_{\Instance,\ClassificationIndex}  \ActiveInstance_{\Instance,\ClassificationIndex}	\leq \CapacityInstances_{\Pop}
\end{equation}

\item Total footprint, latency etc can also be modeled in terms of the $\TrafficFlow$ values


\end{itemize}


==> formulation/simplified/macros_vyas.tex <==
 
\newcommand{\TrafficClass}{\ensuremath{\mathit{class}}}
\newcommand{\TrafficClassIndex}{\ensuremath{\mathit{o}}}
\newcommand{\Traffic}{\ensuremath{\mathit{T}}}
\newcommand{\FootPrint}{\ensuremath{\mathit{F}}}
\newcommand{\Pop}{\ensuremath{\mathit{l}}}
\newcommand{\PopA}{\ensuremath{\mathit{l_\mathit{in}}}}
 \newcommand{\PopB}{\ensuremath{\mathit{l_\mathit{out}}}}
 \newcommand{\Attack}{\ensuremath{\mathit{A}}}
 \newcommand{\NumAttacks}{\ensuremath{\mathit{N}_\Attack}}
 \newcommand{\AttackIndex}{\ensuremath{\mathit{g}}}
 \newcommand{\Detection}{\ensuremath{\mathit{D}}}
 \newcommand{\NumDetection}{\ensuremath{\mathit{N}_\Detection}}
 \newcommand{\DetectionIndex}{\ensuremath{\mathit{d}}}
 \newcommand{\Classification}{\ensuremath{\mathit{C}}}
 \newcommand{\ClassificationIndex}{\ensuremath{\mathit{c}}}
 \newcommand{\NumClassification}{\ensuremath{\mathit{N}_\Classification}}
 \newcommand{\Response}{\ensuremath{\mathit{R}}}
 \newcommand{\ResponseIndex}{\ensuremath{\mathit{r}}}
 \newcommand{\NumResponse}{\ensuremath{\mathit{N}_\Response}}
 \newcommand{\CapacityInstances}{\ensuremath{\mathit{TotalInstances}}}
 \newcommand{\CapacityPerInstance}{\ensuremath{\mathit{Cap}}}
 \newcommand{\DetectionReqd}{\ensuremath{\mathit{ReqD}}}
 \newcommand{\ClassificationReqd}{\ensuremath{\mathit{ReqC}}}
 \newcommand{\ResponseReqd}{\ensuremath{\mathit{ReqR}}}
 \newcommand{\CRChain}{\ensuremath{\mathit{Chain}}}
 
 \newcommand{\ActiveInstance}{\ensuremath{\mathit{h}}}
 \newcommand{\TrafficFlow}{\ensuremath{\mathit{f}}}
 \newcommand{\Instance}{\ensuremath{\mathit{j}}}
 \newcommand{\InstanceToo}{\ensuremath{\mathit{j'}}}
 \newcommand{\InstanceThree}{\ensuremath{\mathit{j''}}}
 \newcommand{\Type}{\ensuremath{\mathit{Type}}}
 \newcommand{\Location}{\ensuremath{\mathit{Loc}}}
 \newcommand{\Load}{\ensuremath{\mathit{Load}}}
 \newcommand{\Chain}{\ensuremath{\mathit{Chain}}}
 \newcommand{\ChainLocation}{\ensuremath{\mathit{k}}}



==> formulation/simplified/requirements.tex <==
\section{System requirements}

Our goal is three-fold:

\begin{itemize}

\item Decide how many {\em instances} of each type of detection, classification, and 
 response modules we need at each location. 

\item Set up the correct flow routing so that the classification and response chain is setup 
 correctly  and that the service chain is implemented correctly

\item Objectives: 
	\begin{itemize}
	\item minimize total latency on impact, 
	\item drop attack traffic as soon as possible,
	\item minimize network congestion as much as possible, 
	\item use as few instances as possible   to minimize total operating cost
	\end{itemize}
\end{itemize}


==> formulation/simplified/system.tex <==
\section{System Model}

\begin{itemize}

\item We have a network with many ingress-egress PoP locations $\PopA$ and
$\PopB$ refer to specific PoPs. 

Let $\Traffic_{\PopA,\PopB}$ denote the total
volume of traffic between the ingress $\PopA$ and the egress $\PopB$. 


\item We have $\NumAttacks$ possible {\em attack traffic classes};
$\Attack_\AttackIndex$ with $\AttackIndex = 1\dots\NumAttacks$   denotes a
specific type of traffic class. Some of these are potential true attacks,
others may be marked as legitimate, while others may be temporarily flagged as
suspicious. These are assumed to be non-overlapping; e.g.,  things like true
syn-flood, potential syn-flood, OK etc.  We say potential because we may not
know how much of it will be true attack until after the required classification
modules have been applied.  We  use the shortcut  $\TrafficClass$ to identify
the combination three-tuple of the ingress-egress-type and the shortcut index
$\TrafficClassIndex$ to capture a specific three-tuple
$\langle\PopA,\PopB,\AttackIndex\rangle$

 Let $\Traffic_{\PopA,\PopB,\AttackIndex}$
denote the total volume of traffic of type $\AttackIndex$ from ingress $\PopA$
to egress $\PopB$.  


\item We have $\NumDetection$ possible {\em attack detection} modules and
$\Detection_\DetectionIndex$ with $\DetectionIndex \in 1\dots\NumDetection$
denotes one specific type of detection module


\item We have $\NumClassification$ possible {\em attack classification} modules
and $\Classification_\ClassificationIndex$ with $\ClassificationIndex \in
1\dots\NumClassification$ denotes one specific type of classification module

\item We have $\NumResponse$ possible {\em attack response} modules 
 and $\Response_\ResponseIndex$ with $\ResponseIndex \in 1\dots\NumResponse$ 
denoting one specific type of response module

\item   We assume we have some pre-provisioned  total capacity  at each
location $\Pop$.  Let $\CapacityInstances_{\Pop}$ denote the total provisioned
capacity in terms of the {\em number of instances} of $\Pop$.

 Each instance will be assigned for some specific role; e.g., for detection
module $\DetectionIndex$, classification module $\ClassificationIndex$ and
response module $\ResponseIndex$ respectively.

 We assume each {\em instance} (say a virtual appliance) of a particular type
if deployed has a fixed  total   capacity;
$\CapacityPerInstance_\DetectionIndex$,
$\CapacityPerInstance_\ClassificationIndex$,
$\CapacityPerInstance_\ResponseIndex$ denotes the volume of traffic  each
instance can handle.

\item We use the generic index $\Instance$ to refer to one of these virtual 
 instances running somewhere. $\Type_\Instance$ identifies the type of 
 the instance and $\Location_\Instance$  gives its location 


\item We assume that {\em all traffic} from  $\Traffic_{\PopA,\PopB}$ undergoes
some detection logic. The specific modules may be different.  We use indicator
values $\DetectionReqd_{\PopA,\PopB,\DetectionIndex}$ to denote if the traffic
from $\PopA$ to $\PopB$ requires the detection module $\DetectionIndex$.

%Let
%$\FootPrint_{\PopA,\PopB,\DetectionIndex}$ denote the per-traffic unit
%footprint cost of running the detection module $\DetectionIndex$ on traffic
%from $\PopA$ to $\PopB$. If some detection module is not required,
% then the footprint is simply set to zero.

\item However only the potential attack traffic undergoes the required
classification and response modules.
%  Let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ denote the cost
%of running the classification module $\ClassificationIndex$ for the potential
%attack traffic of type $\AttackIndex$ from  $\PopA$ to $\PopB$. Again this is
%zero if this type of analysis is not required.  Similarly, let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ denote the cost  of
%running the response module $\ResponseIndex$ for the potential attack traffic
%of type $\AttackIndex$ from  $\PopA$ to $\PopB$
% Similarly to the detection case, we use indicator values
%$\ClassificationReqd_{\TrafficClassIndex,\ClassificationIndex}$ and
%$\ResponseReqd_{\TrafficClassIndex,\ResponseIndex}$ to denote if the
%corresponding classification and response modules are required for the 
% specific  $\TrafficClass$ $\TrafficClassIndex$.
%\item
 There is  a specific {\em chaining} of modules that need to be applied
for each $\TrafficClassIndex$. Let $\Chain_{\TrafficClassIndex}$ denote the
specific chain of modules required in terms of the required
classification/response capabilities; i.e., each element in the chain 
 is some $\ClassificationIndex$ or $\ResponseIndex$.   We use $|\Chain_{\TrafficClassIndex}|$
to denote the length of the chain, and
$\Chain_{\TrafficClassIndex}[\ChainLocation]$ to denote the module function at
the $\ChainLocation^\mathit{th}$ point in the chain.  Let
$\Type_{\Chain_{\TrafficClassIndex}[\ChainLocation]}$  denote the type of
module at this point in the chain.
 

\end{itemize}





==> formulation/system.tex <==
\section{System Model}

\begin{itemize}

\item We have a network with many ingress-egress PoP locations $\PopA$ and
$\PopB$ refer to specific PoPs. 

Let $\Traffic_{\PopA,\PopB}$ denote the total
volume of traffic between the ingress $\PopA$ and the egress $\PopB$. 


\item We have $\NumAttacks$ possible {\em attack traffic classes};
$\Attack_\AttackIndex$ with $\AttackIndex = 1\dots\NumAttacks$   denotes a
specific type of traffic class. Some of these are potential true attacks,
others may be marked as legitimate, while others may be temporarily flagged as
suspicious. These are assumed to be non-overlapping; e.g.,  things like true
syn-flood, potential syn-flood, OK etc.  We say potential because we may not
know how much of it will be true attack until after the required classification
modules have been applied.  We  use the shortcut  $\TrafficClass$ to identify
the combination three-tuple of the ingress-egress-type and the shortcut index
$\TrafficClassIndex$ to capture a specific three-tuple
${\PopA,\PopB,\AttackIndex}$

 Let $\Traffic_{\PopA,\PopB,\AttackIndex}$
denote the total volume of traffic of type $\AttackIndex$ from ingress $\PopA$
to egress $\PopB$.  


\item We have $\NumDetection$ possible {\em attack detection} modules and
$\Detection_\DetectionIndex$ with $\DetectionIndex \in 1\dots\NumDetection$
denotes one specific type of detection module


\item We have $\NumClassification$ possible {\em attack classification} modules
and $\Classification_\ClassificationIndex$ with $\ClassificationIndex \in
1\dots\NumClassification$ denotes one specific type of classification module

\item We have $\NumResponse$ possible {\em attack response} modules 
 and $\Response_\ResponseIndex$ with $\ResponseIndex \in 1\dots\NumResponse$ 
denotes one specific type of response module

\item   We assume we have some pre-provisioned  total capacity  for each type
of detection, response, classification module at each location $\Pop$.  Let
$\CapacityInstances_{\Pop,\DetectionIndex}$,
$\CapacityInstances_{\Pop,\ClassificationIndex}$,
$\CapacityInstances_{\Pop,\ResponseIndex}$ respectively denote the total
provisioned capacity in terms of the {\em number of instances} of $\Pop$ for
detection module $\DetectionIndex$, classification module
$\ClassificationIndex$ and response module $\ResponseIndex$ respectively.

\item  We assume each {\em instance} (say a virtual appliance) of a particular
type  if deployed has a fixed  total   capacity;
$\CapacityPerInstance_\DetectionIndex$,
$\CapacityPerInstance_\ClassificationIndex$,
$\CapacityPerInstance_\ResponseIndex$ denotes the volume of traffic  each
instance can handle.

\item We use the generic index $\Instance$ to refer to one of these module
 instances running somewhere. $\Type_\Instance$ identifies the type of 
 the instance and $\Location_\Instance$  gives its location 


\item We assume that {\em all traffic} from  $\Traffic_{\PopA,\PopB}$ undergoes
some detection logic. The specific modules may be different.  We use indicator
values $\DetectionReqd_{\PopA,\PopB,\DetectionIndex}$ to denote if the traffic
from $\PopA$ to $\PopB$ requires the detection module $\DetectionIndex$.

%Let
%$\FootPrint_{\PopA,\PopB,\DetectionIndex}$ denote the per-traffic unit
%footprint cost of running the detection module $\DetectionIndex$ on traffic
%from $\PopA$ to $\PopB$. If some detection module is not required,
% then the footprint is simply set to zero.

\item However only the potential attack traffic undergoes the required
classification and response modules.
%  Let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ denote the cost
%of running the classification module $\ClassificationIndex$ for the potential
%attack traffic of type $\AttackIndex$ from  $\PopA$ to $\PopB$. Again this is
%zero if this type of analysis is not required.  Similarly, let
%$\FootPrint_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ denote the cost  of
%running the response module $\ResponseIndex$ for the potential attack traffic
%of type $\AttackIndex$ from  $\PopA$ to $\PopB$
 Similarly to the detection case, we use indicator values
$\ClassificationReqd_{\PopA,\PopB,\AttackIndex,\ClassificationIndex}$ and
$\ResponseReqd_{\PopA,\PopB,\AttackIndex,\ResponseIndex}$ to denote if the
corresponding classification and response modules are required for the 
 potential attack traffic from $\PopA$ to $\PopB$.

\item There might also be a specific {\em chaining} of modules that need 
 to be applied for each $ \PopA,\PopB,\AttackIndex$ tuple. Let $\Chain_{\PopA,\PopB,\AttackIndex}$
 denote the specific chain of modules required in terms of the required classification/response 
 capabilities.   We use $|\Chain_{\PopA,\PopB,\AttackIndex}|$ to denote the length 
 of the chain, and $\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]$ to denote the module 
 function at the $\ChainLocation^\mathit{th}$ point in the chain.
 Let $\Type_{\Chain_{\PopA,\PopB,\AttackIndex}[\ChainLocation]}$  denote the type 
 of module at this point in the chain.
 

\end{itemize}





==> outline.tex <==
\section{Introduction}

\begin{packeditemize}

\item networks' complexity makes them error prone. network operators (a.k.a. masters 
of complexity) need to make sure policies are enforced despite all this complexity. 
this is difficult today and the process is mostly manual and error-prone.

\item to verify successful enforcement network policies, it is necessary to conduct 
verification as close to the wire as possible. to test the network in a live manner, 
we need to inject carefully selected test traffic into the data plane and verify the
observed behavior of the data plane against the expected behavior mandated by the 
policies.

\item today's realistic network testing scenarios fall outside the purvey of the 
existing work in that both policy requirement and data plane elements are stateful 
and dynamic: 
(1) service chaining policies~\cite{ietfnsc} are by structure stateful and dynamic (e.g., send traffic
to the heavy IPS only if it has triggered an alarm on the light IPS), (2) many 
middleboxes that are widely used expose stateful and dynamic behavior
(e.g., stateful firewall, providing cached response by a proxy). These two dimensions
mandate test requirements that go beyond what existing solutions offer.

\item given the overarching vision of CAD for networks, we have developed \Name, 
a framework to efficiently test realistic data plane despite the above challenges. given 
a set of network policy requirements, first, \Name helps model the data plane as a finite state 
machine to facilitate formulating the test goals and make the test process intuitive. 
Then \Name generates test traffic that is carefully chosen as to efficiently explore 
the ``state space'' of data plane. It then monitors network-wide behavior and validates 
it against the policies.

\item we make three contributions:

\begin{packeditemize}

\item \mypara{Modeling the data plane} we provide a framework to model individual data 
plane elements (e.g., firewalls, proxies) such that they can be composed with each other, 
yielding a \emph{data plane model} as a finite state-machine. this is useful for 
two reasons: (1) it helps us define and tackle the problem of testing the data plane in 
systematic and yet intuitive way, (2) data plane model be useful for activities other 
than test (e.g., XXX).

\item \mypara{Planning test traffic} given a set of intended network-wide policies, we 
identify and implement the key components of a network-wide test framework. this involves 
formulating a test plan (i.e., where and when to inject what test traffic) that strikes 
a balance between the \emph{efficiency} and \emph{coverage} of test in realistic scenarios.

\item \mypara{Interpreting test results} \Name then monitors the behavior of the data 
plane w.r.t. the injected test traffic and infers whether it complies with our intended 
policies. in so doing, we have overcome the challenge of mutual \emph{interference} between 
regular network traffic (e.g., from users, departments) and test traffic, w.r.t. both 
performance and correctness.

\end{packeditemize}

\end{packeditemize}



\section{Motivation}

\begin{packeditemize}

\item to bring a conceptual framework to motivation, maybe put a symbolic 2D plane figure 
here. the X-axis is policy space (i.e., things we want to enforce) and the Y-axis is data 
plane state space (i.e., what possible states the entire data plane can be in at any given 
time). on each axis there are a set of regions that we "care" about. the intersection(s) of 
them give(s) the region(s) that we need to focus on. give an example of how this region is
identified. then we can discuss there is no framework that helps us systematically these 
regions of concern.

\end{packeditemize}

\begin{packeditemize}

\item example 1---should encompass stateful/dynamic policy and stateful/dynamic data plane

\item example 2---should encompass stateful/dynamic policy and stateful/dynamic data plane

\item strawman solutions:

\begin{packeditemize}

\item static verification~\cite{hsa, veriflow, netplumber}

\item test packet generation~\cite{atpg}

\item existing firewall/IPS testing tools~\cite{}

\item testing control plane~\cite{nice,tshoot_sigcomm14}

\item policy steering tools~\cite{simplesigcomm, flowtags_nsdilong}

\end{packeditemize}

\item we refute each of them in (a subset of) these four dimensions: 

\begin{packeditemize}

\item failing to capture stateful/dynamic policies

\item failing to capture stateful/dynamic data plane elements

\item failing to capture data plane-level problems

\item lack of network-wide testing
\end{packeditemize}

\end{packeditemize}


\section{\Name Overview}

\subsection{System architecture}

\begin{packeditemize}

\item describe the overall scenario.

\item make it clear that we are not verifying data plane implementation's correctness 
(as opposed to epfl14). we are testing whether the policies are enforced correctly.

\item walk through the solution components:

\begin{packeditemize}

\item data-plane modeler

\item test traffic planner

\item monitoring and validation engines

\end{packeditemize}

\end{packeditemize}

\subsection{End-to-end example}

\begin{packeditemize}

\item highlight why doing something trivial in each stage is not enough.

\end{packeditemize}


\section{Modeling Data Plane}

\begin{packeditemize}

\item show strawman solutions don't solve what this section achieves.(see questions 2 and 3 below.)

\item Question 1: why do we model the data plane? existing state of affairs is too 
messy. e.g., a real middlebox code base is too big and too complex and 
not well-documented. modeling them is a way of:

\begin{packeditemize}

\item  taming this complexity to enable systematic testing of the data plane

\item help network operators understand the stateful and dynamic behavior of the 
data plane

\end{packeditemize}

\item Question 2: strawman solutions for not doing modeling altogether?

\begin{packeditemize}

\item just use the policy spec (e.g., the \DPG) to test the network.

\begin{packeditemize}

\item this is not sufficient: without accounting for the stateful nature of the data plane, we have
no systematic way of knowing what we are actually testing. for example, we may inject some test traffic
and see that it succeeds. however, we don't know under what state this specific test has succeeded (i.e.,
lack of coverage, and even worse, not knowing what we have covered).

\end{packeditemize}


\end{packeditemize}

\item Question 3: strawman solutions for modeling the data plane?

\begin{packeditemize}

\item located packet/HSA/transfer function. this approach cannot capture a few important aspects of real data planes:

\begin{packeditemize}

\item stateful elements: HSA assumes a transfer function is just a function of input packet, not the possible \DPF's state. 

\item HSA assumes the unit of processing is the same all through the data path (e.g., $f_1$, $f_2$, $f_3$,\dots each process input packet $X$ and throw out $f_3(f_2(f_1(X)))$).
The reality is $f_1$ (a router) and $f_2$ (a packet filter) may act on a per-packet basis, but $f_3$ (a proxy) may process HTTP sessions. In other words, the \emph{operational 
semantics} and \emph{time granularity} of different functions may be different, which makes their composition non-trivial. 


\end{packeditemize}
\end{packeditemize}

\item Question 4: many ways of modeling a system. what kind of model do we need?

\begin{packeditemize}

\item capture the stateful and dynamic aspects of the data plane that affect policy correctness

\item intuitive and easy to understand by human operators

\end{packeditemize}


\item Question 5: modeling assumptions and goals?

\begin{packeditemize}

\item the middlebox implementation is ``correct'' (i.e., no crashed, unintended 
infinite loops, memory leaks). 

\item the goal of the modeling activity is to capture and visualize. stateful and 
dynamic traffic processing behaviors of each middlebox.

\item finally we glue together the individual element models according to the topology 
and create a network-wide data plane model.

\end{packeditemize}


\item Question 6: access to middlebox code?

\begin{packeditemize}

\item yes. ``white-box modeling''

\item no. ``blackbox-box modeling''

\end{packeditemize}

\item one tricky case is non-deterministic behavior of NATs etc. maybe we can use NFAs in this case with $\epsilon$ transitions. at least it can show
us what kind of things can go wrong in the data plane.

\end{packeditemize}




\section{Test Traffic Planning and Injection}

\begin{packeditemize}

\item show strawman solutions don't solve what this section achieves.

\item Input: topology, data plane model, policies

\item Output: test plan which specifies what test packet to inject from where and when

\item challenges: 

\begin{packeditemize}

\item how to make sure the test traffic covers the policy space? 

\item given a cap for test traffic volume, what states are more important to cover?

\item how to accommodate practical network constraints (e.g., i can use only a subset of hosts to 
inject test traffic; or, my test traffic should not be of a protocol that a firewall will drop)


\end{packeditemize}

\end{packeditemize}

\section{Monitoring and Validation}
\subsection{Monitoring}

\begin{packeditemize}

\item show strawman solutions don't solve what this section achieves.

\item Input: test plan

\item Output: what can i infer wrt to policies? with what confidence?

\item Goal: capture enough traffic to make inference possible

\item challenges: 

\begin{packeditemize}

\item traffic log size. should sample in a meaningful way.

\item choice of monitoring nodes can be limited

\end{packeditemize}

\end{packeditemize}

\subsection{Validation}
\begin{packeditemize}

\item Input: policies, topology, captured monitored traffic, models

\item Output: what can i infer wrt to policies? with what confidence?

\item challenges: 

\begin{packeditemize}

\item ``performance interference'' with regular traffic: don't want to congest the network with test traffic

\item ``correctness interference'' with regular traffic: dint want to let the test traffic semantically make thing 
wrong for the regular traffic or vice versa (e.g., a counting up IPS)

\end{packeditemize}

\end{packeditemize}


\section{Diagnosis---on hold}

\section{Evaluations}

\subsection{Evaluation Questions}

\begin{packeditemize}

\item Q1---Can we model the data plane correctly?

\begin{packeditemize}

\item element model validation---have we modeled each data plane element correctly?

\begin{packeditemize}

\item introduce bugs (w.r.t. policies) into code and see if that is captured in the model

\item use test traces and compare the output of the code and the model on test trace

\end{packeditemize}

\item data plane model validation---have we modeled the entire data plane correctly?

\begin{packeditemize}

\item in a given network test trace, is there any discrepancy between the data plane and the model w.r.t. policies?

\end{packeditemize}

\end{packeditemize}


\item Q2---Can we model the data plane efficiently?

\begin{packeditemize}

\item how long does it take to synthesize data plane model? is it a function of LoC?

\item we need to somehow show the trade-off between model's size and usability. maybe belongs
to the following questions.

\end{packeditemize}

\item Q3---What kind of bugs can \Name capture? ---the 
metrics here is coverage (i.e., what fraction of bugs \Name find.)

\begin{packeditemize}

\item known correctness bugs

\item new correctness bugs

\item synthesized correctness bugs

\item performance bugs

\end{packeditemize}

\item Q4---Can \Name effectively cope with interference?

\begin{packeditemize}

\item correctness interference

\item performance interference

\end{packeditemize}

\item Q5---What is the performance of \Name?

\begin{packeditemize}

\item how long does it take to test the policies? 

\begin{packeditemize}

\item break it down to its states: (1) planning, (2) injection, (3) monitoring, (4) inference

\end{packeditemize}

\item memory and bandwidth overhead

\end{packeditemize}

\item Q6---Does \Name scale?

\begin{packeditemize}

\item run time as a function of policy complexity, and as a function of network topology

\end{packeditemize}

\end{packeditemize}

\subsection{Testbed}

\input{concerns}



==> puttogether.tex <==
\section{Putting it Together}
\label{sec:puttingittogether}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Example Use Case: UDP Flood Attack}

Next we present an example use case of \Name under a UDP flood attack 
scenario.

\begin{figure*}[t!]
\centering
\subfloat[Classification at time $t_1$.]
{
%\vspace{-0.6cm}
\includegraphics[width=250pt]{figs/overview_usecase_part1of3.pdf}
\label{fig:stage1}
}
\hspace{1.1cm}
\subfloat[Analysis and response at time $t_2$.]
{
%\vspace{-0.6cm}
\includegraphics[width=250pt]{figs/overview_usecase_part2of3.pdf}
\label{fig:stage2}
}
\hspace{.1cm}

\subfloat[Response only at time $t_3$.]
{
%\vspace{-0.6cm}
\includegraphics[width=250pt]{figs/overview_usecase_part3of3.pdf}
\label{fig:stage3}
}
\caption{Example use case of \Name in case of UDP flood attack.}
\vspace{-0.5cm}
\label{fig:udp_usecase_overview}
\end{figure*}


\emph{Step 0 --- Initialization:} The sampling scheme can be s-flow as
supported by ISP switches with a certain sampling rate.

\emph{Step 1 --- Classification (C):} The classification function receives 
meta-data of sampled traffic. After getting enough meta-data, at time 
\emph{$t_1$} it infers that input traffic that matches the pattern 
``\emph{dstIP=192.168.0.0/16} and \emph{proto=UDP}'' is UDP attack.
It informs the controller of this result. (see Figure~\ref{fig:stage1}.)

\emph{Step 2 --- Analysis (A):} If not already launched, the controller 
launches the analysis and response modules for UDP attack as 
per policies library. These are denoted by $A_{UDP}$ and $R_{UDP}$ 
in Figure~\ref{fig:stage2}, respectively. 

The controller configures switches to use tag values
for traffic steering. In particular, it configures ingress switches 
to mark input traffic that matches ``\emph{dstIP=192.168.0.0/16} 
and \emph{proto=UDP}'' with tag value 1. Other on-path 
switches are configured to forward packets with tag=1 to 
$A_{UDP}$.

$A_{UDP}$ performs in depth analysis of the suspicious 
traffic (as inferred by classification) and finds out that 
\emph{dstIP=192.168.0.0/17} is indeed UDP attack, but 
\emph{dstIP=192.168.128.0/17} is benign.\footnote{As we will
see in~\S\ref{sec:XXX}, the analysis modules find patterns at a 
5-tuple level. For ease of presentation in this high-level example, 
we show /17 rules.} 
$A_{UDP}$ 
tags its outgoing traffic with tag values 2 and 3, respectively.

The controller has already configured switches to steer
traffic with $tag=2$ to response module $R_{UDP}$ and traffic
with $tag=3$ to the customer.


\emph{Step 3 --- Response (R):} In this example, the response 
module $R_{UDP}$ simply drops attack traffic.

\Name acts proactively whenever possible. In this example,
as shown in Figure~\ref{fig:stage3}, the controller uses the information
reported by $A_{UDP}$ to install fine-grained tagging rules at the 
ingress at time $t_3$. In particular, from this time on, the ingress 
switch marks \emph{dstIP=192.168.0.0/17} with $tag=2$ and 
\emph{dstIP=192.168.128.0/17} with $tag=3$. Other switches 
are configured to steer such traffic correctly as shown in 
Figure~\ref{fig:stage3}. The advantage here is to bypass $A_{UDP}$.

\subsection{Putting it together}
use toby's figure that explains everything.





==> todo.tex <==
\section{TODOs}
\begin{itemize}

 \item find anecdotes for section 2
  
\item we should say somewhere that if attack traffic is not detected as attack, the ISP 
simply rate limits all traffic to at least provide legitimate and attack traffic with fairness.

  
\end{itemize}


